Foundations of Multisensory Artificial Intelligence

Building multisensory AI systems that learn from multiple sensory inputs such as text, speech, video, real-world sensors, wearable devices, and medical data holds great promise for impact in many scientific areas with practical benefits, such as in supporting human health and well-being, enabling multimedia content processing, and enhancing real-world autonomous agents. By synthesizing a range of theoretical frameworks and application domains, this thesis aims to advance the machine learning foundations of multisensory AI. In the first part, we present a theoretical framework formalizing how modalities interact with each other to give rise to new information for a task. These interactions are the basic building blocks in all multimodal problems, and their quantification enables users to understand their multimodal datasets, design principled approaches to learn these interactions, and analyze whether their model has succeeded in learning. In the second part, we study the design of practical multimodal foundation models that generalize over many modalities and tasks, which presents a step toward grounding large language models to real-world sensory modalities. We introduce MultiBench, a unified large-scale benchmark across a wide range of modalities, tasks, and research areas, followed by the cross-modal attention and multimodal transformer architectures that now underpin many of today's multimodal foundation models. Scaling these architectures on MultiBench enables the creation of general-purpose multisensory AI systems, and we discuss our collaborative efforts in applying these models for real-world impact in affective computing, mental health, cancer prognosis, and robotics. Finally, we conclude this thesis by discussing how future work can leverage these ideas toward more general, interactive, and safe multisensory AI.

==> 02_rus/figures/annotation.tex <==
\begin{figure*}[tbp]
\centering
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{02_rus/figures/direct.pdf}
\end{subfigure}\vspace{2mm}\\%
\vspace{-2mm}
\caption{We show a sample user interface for annotating information decomposition into redundancy, uniqueness, and synergy, which we give to $3$ annotators each to obtain agreeing and reliable judgments of each interaction for real-world multimodal datasets.}
\label{fig:annotations}
\vspace{-2mm}
\end{figure*}

==> 02_rus/figures/overview.tex <==
\begin{figure}[tbp]
\centering
\vspace{-6mm}
\includegraphics[width=0.9\linewidth]{02_rus/figures/overview_fig_fig.pdf}
\vspace{-2mm}
\caption{The \name\ framework formalizes the nature of feature interactions for a task. Through our proposed scalable estimators for \textit{redundancy}, \textit{uniqueness}, and \textit{synergy}, we demonstrate its usefulness towards quantifying multimodal datasets, model predictions, and model selection.}
\label{fig:overview}
\vspace{-4mm}
\end{figure}

==> 02_rus/figures/robust.tex <==
\begin{figure}[tbp]
\centering
\vspace{-0mm}
\includegraphics[width=0.8\linewidth]{02_rus/figures/unimodal_robust.pdf}
\vspace{-2mm}
\caption{We find high correlation ($0.62$) between the performance drop when $X_i$ is missing and the model's $U_i$ value: high $U_i$ coincides with large performance drops, but low $U_i$ can also lead to performance drops. The latter can be further explained by the presence of large $R$ and $S$ values despite low $U_i$ which also causes performance drops.}
\label{fig:robust}
\vspace{-2mm}
\end{figure}

==> 02_rus/tables/agreement.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{1mm}
\caption{Annotator agreement and average confidence scores of human annotations of \name\ values for real-world multimodal datasets.}
\centering\begin{tabular}{l|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{Agreement} & \multicolumn{4}{c}{Confidence} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
Human & $0.72$ & $0.68$ & $0.70$ & $0.72$ & $4.36$ & $4.35$ & $4.27$ & $4.46$ \\
\hline \hline
\end{tabular}

\vspace{-0mm}
\label{tab:agreement}
\end{table}

==> 02_rus/tables/compare.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-0mm}
\caption{Comparison between \esta\ and \estb\ on selected real-world datasets.}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{AV-MNIST}} & \multicolumn{4}{c}{\textsc{Push i,c}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\esta & $0.10$ & $0.97$ & $0.03$ & $0.08$ & $0.24$ & $0.03$ & $0.06$ & $0.04$ \\
\estb & $0.40$ & $1.04$ & $0.04$ & $0.16$ & $0.75$ & $1.79$ & $0.03$ & $0.08$ \\
\hline \hline
\end{tabular}
\label{tab:comp_batch}
\end{table*}

==> 02_rus/tables/datasets_full.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\vspace{-0mm}
\caption{Full results on estimating \name\ on real-world MultiBench~\citep{liang2021multibench} datasets. Many of the estimated interactions align well with dataset construction (e.g., \textsc{MUStARD} for sarcasm) and unimodal performance (e.g., \textsc{MIMIC} and \textsc{AV-MNIST}). On QA~\cite{antol2015vqa} datasets, synergy is consistently the highest.}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{AV-MNIST}} & \multicolumn{4}{c|}{\textsc{ENRICO}} & \multicolumn{4}{c|}{\textsc{VQA 2.0}} & \multicolumn{4}{c}{\textsc{CLEVR}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\esta\ & $0.10$ & $\bm{0.97}$ & $0.03$ & $0.08$ & $\bm{0.73}$ & $0.38$ & $0.53$ & $0.34$ & $0.79$ & $0.87$ & $0$ & $\mathbf{4.92}$ & $0.55$ & $0.48$ & $0$ & $\mathbf{5.16}$\\
\hline \hline
\end{tabular}

\vspace{2mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{MIMIC}} & \multicolumn{4}{c|}{\textsc{UR-FUNNY a,t}} & \multicolumn{4}{c|}{\textsc{UR-FUNNY v,t}} & \multicolumn{4}{c}{\textsc{UR-FUNNY v,a}}\\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\estb\ & $0.05$ & $\bm{0.17}$ & $0$ & $0.01$ & $0.02$ & $0$ & $\bm{0.08}$ & $0.07$ & $0.06$ & $0$ & $0.04$ & $\bm{0.11}$ & $0.02$ & $0.04$ & $0$ & $\bm{0.06}$ \\
\hline \hline
\end{tabular}

\vspace{2mm}

\begin{tabular}{l|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{MOSEI a,t}} & \multicolumn{4}{c|}{\textsc{MOSEI v,t}} & \multicolumn{4}{c}{\textsc{MOSEI v,a}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\estb\ & $0.22$ & $0.04$ & $0.09$ & $\bm{0.13}$ & $0.30$ & $\bm{0.70}$ & $0$ & $0$ & $0.26$ & $\bm{0.74}$ & $0$ & $0$ \\
\hline \hline
\end{tabular}

\vspace{2mm}

\begin{tabular}{l|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{MUStARD a,t}} & \multicolumn{4}{c|}{\textsc{MUStARD v,t}} & \multicolumn{4}{c}{\textsc{MUStARD v,a}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\estb\ & $0.14$ & $0.01$ & $0.01$ & $\bm{0.37}$ & $0.14$ & $0.02$ & $0.01$ & $\bm{0.34}$ & $0.14$ & $0.01$ & $0.01$ & $\bm{0.20}$ \\
\hline \hline
\end{tabular}


\vspace{-0mm}
\label{tab:datasets_full}
\end{table*}

==> 02_rus/tables/datasets_qa.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-0mm}
\caption{Estimating \name\ on QA~\cite{antol2015vqa} datasets with both \esta\ and \estb\ estimators. Synergy is consistently the highest and both estimators return \name\ values that are consistent relative to each other.}
\centering
\footnotesize
\vspace{-0mm}

\begin{tabular}{l|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{VQA 2.0}} & \multicolumn{4}{c}{\textsc{CLEVR}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
% \esta & $7.89\times10^{-4}$  & $8.73\times10^{-4}$ & $0$ & $4.92\times10^{-3}$ &  $5.51\times10^{-4}$  & $4.80\times10^{-4}$ & $8.47\times10^{-14}$ & $5.16\times10^{-3}$  \\
\esta & $0.79$ & $0.87$ & $0$ & $\mathbf{4.92}$ & $0.55$ & $0.48$ & $0$ & $\mathbf{5.16}$\\
\estb & $0.10$ & $0.14$ & $0.09$ & $\mathbf{0.16}$ & $0.01$ & $0.01$ & $0.01$ & $\mathbf{0.03}$\\
Human & $0.23$ & $0$ & $0$ & $\mathbf{4.80}$ & $0$ & $0$ & $0$ & $\mathbf{5.00}$ \\
\hline \hline
\end{tabular}

\vspace{-2mm}
\label{tab:datasets_qa}
\end{table}

==> 02_rus/tables/gmm.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-2mm}
\caption{Results on estimating \name\ across different GMM}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{4}{c|}{\textsc{General}} & \multicolumn{16}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{EF}} & \multicolumn{4}{c|}{\textsc{Additive}} & \multicolumn{4}{c|}{\textsc{Agree}} & \multicolumn{4}{c|}{\textsc{Align}} & \multicolumn{4}{c}{\textsc{SSL}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
ur-funny {a,t} & 0.02 & 0 & 0.02 & 0.06 & 0.02 & 0 & 0.02 & 0.15 & 0.02 & 0 & 0.02 & 0.05 & 0.02 & 0 & 0.02 & 0.06 & &  &  & \\
ur-funny {v,t} & 0.05 & 0.01 & 0 & 0.17 & 0.11 & 0.08 & 0 & 0.17 & 0.02 & 0.04 & 0 & 0.24 & 0.02 & 0 & 0.02 & 0.15 & &  &  & \\
ur-funny {v,a} & 0.01 & 0.27 & 0 & 0.19 & 0.03 & 0 & 0.02 & 0.15 &  0.02 & 0 & 0.02 & 0.15 & 0.12 & 0.05 & 0.01 & 0.19 & &  &  & \\
mosei t,a & 0.03 & 0 & 0.05 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0 & 0.02 & & &  &\\
% & $9.46\times10^{-12}$ & $-1.17\times10^{-17}$ & $5.57\times10^{-17}$ & $-9.46\times10^{-12}$
mosei t,v & 0 & 0 & 0 & 0 & 0.02 & 0 & 0.02 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.03 & 0 & 0 & 0.03 & & &  &\\
mosei a,v & 0 & 0 & 0 & 0 & 0.08 & 0.01 & 0 & 0.02 & 0.07 & 0 & 0 & 0.02 & 0.13 & 0 & 0.02 & 0.02 & & &  &\\
mimic & 0.01 & 0.27 & 0 & 0 & 0.01 & 0.27 & 0 & 0 & 0.01 & 0.27 & 0 & 0 & 0.01 & 0.28 & 0 & 0 & &  &  &   \\
avmnist \\
push \\
enrico & 0.71 & 0.34 & 0.44 & 0.38 & 0.69 & 0.28 & 0.39 & 0.35
 & & & &  & 0.40 & 0.30 & 0.52 & 0.75 & &  &  &  \\
vqa \\
clevr \\
Average & \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{4}{c|}{\textsc{General}} & \multicolumn{16}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{EF}} & \multicolumn{4}{c|}{\textsc{Additive}} & \multicolumn{4}{c|}{\textsc{Agree}} & \multicolumn{4}{c|}{\textsc{Align}} & \multicolumn{4}{c}{\textsc{SSL}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
$(z_c)$ & 0.47 & 0.01 & 0.01 & 0.04 & 0.56 & 0.01 & 0.01 & 0.03 & 0.56 & 0.01 & 0 & 0.03 & 0.57 & 0.01 & 0.01 & 0.03 \\
$(z_1)$ & 0 & 0.41 & 0 & 0.04 & 0.01 & 0.02 & 0 & 0.06 & 0.07 & 0.44 & 0 & 0.02 & 0.02 & 0.13 & 0 & 0.08 \\
$(z_2)$ & 0.01 & 0 & 0.47 & 0.04 & 0.01 & 0 & 0.58 & 0.01 & 0.01 & 0 & 0.59 & 0.01 & 0.01 & 0 & 0.59 & 0.01 \\
$(z_1,z_2)$ & 0.15 & 0.02 & 0 & 0.29 & 0.1 & 0 & 0.19 & 0.25 & 0.1 & 0 & 0.18 & 0.26 & 0.1 & 0 & 0.17 & 0.27 \\
$(z_1^*,z_2^*,z_c^*)$ & 0.22 & 0 & 0.07 & 0.15 & 0.29 & 0 & 0.16 & 0.11 & 0.28 & 0 & 0.15 & 0.12 & 0.3 & 0 & 0.15 & 0.13 \\
$(z_1,z_2^*,z_c^*)$ & 0.16 & 0.15 & 0 & 0.15 & 0.2 & 0 & 0.06 & 0.09 & 0.13 & 0 & 0.11 & 0.09 & 0.18 & 0 & 0.06 & 0.09 \\
$(z_1,z_2,z_c^*)$ & 0.16 & 0.05 & 0 & 0.25 & 0.15 & 0 & 0.25 & 0.13 & 0.15 & 0 & 0.22 & 0.13 & 0.16 & 0 & 0.25 & 0.11 \\
$(z_1^*,z_2^*,z_c)$ & 0.25 & 0.03 & 0 & 0.14 & 0.44 & 0 & 0.04 & 0.1 & 0.41 & 0 & 0.08 & 0.07 & 0.42 & 0 & 0.07 & 0.1 \\
$(z_2^*,z_c^*)$ & 0.19 & 0 & 0.12 & 0.06 & 0.2 & 0 & 0.27 & 0.03 & 0.22 & 0 & 0.32 & 0.02 & 0.18 & 0 & 0.32 & 0.03 \\
$(z_2^*,z_c)$ & 0.26 & 0 & 0.12 & 0.05 & 0.37 & 0 & 0.18 & 0.04 & 0.34 & 0 & 0.17 & 0.04 & 0.35 & 0 & 0.19 & 0.04 \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{16}{c|}{\textsc{Synergy}} & \multicolumn{8}{c}{\textsc{Unique}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{Elem}} & \multicolumn{4}{c|}{\textsc{Outer}} & \multicolumn{4}{c|}{\textsc{MI}} & \multicolumn{4}{c|}{\textsc{MulT}} & \multicolumn{4}{c|}{\textsc{Lower}} & \multicolumn{4}{c}{\textsc{Rec}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
ur-funny t,a & 0.01 & 0 & 0.03 & 0.05 & 0.01 & 0 & 0.02 & 0.05 & 0.01 & 0 & 0.03 & 0.04 & & & & & 0.02 & 0 & 0.01 & 0.14 & 0.01 & 0 & 0.02 & 0.04 \\
ur-funny t,v & 0.02 & 0.01 & 0 & 0.16 & 0.03 & 0.01 & 0 & 0.14 & 0.04 & 0.02 & 0 & 0.14 & & & & & 0.04 & 0 & 0.01 & 0.15 & 0.03 & 0.01 & 0 & 0.17 \\
ur-funny a,v & 0.03 & 0.13 & 0 & 0.16 & 0.02 & 0.15 & 0 & 0.15 & 0.02 & 0.23 & 0 & 0.15 & & & & & 0.02 & 0.15 & 0 & 0.19 & 0.05 & 0.08 & 0 & 0.20 \\
mosei t,a & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0.02 & 0.02 & & & & & 0.02 & 0 & 0.04 & 0.02 \\
mosei t,v & 0.01 & 0 & 0.04 & 0.03 & 0.01 & 0 & 0.04 & 0.03 & 0.03 & 0 & 0.03 & 0.03 & & & & & 0.02 & 0 & 0.04 & 0.03 & &  &\\
mosei a,v & 0.03 & 0.02 & 0 & 0.02 & 0.02 & 0.01 & 0 & 0.01 & 0.03 & 0.01 & 0 & 0.02 & & & & & 0.02 & 0.01 & 0 & 0.01 \\
mimic & 0.04 & 0.24 & 0 & 0.01 & 0 & 0.28 & 0 & 0.01 & 0.02 & 0.26 & 0 & 0.01 & & & & & 0.01 & 0.28 & 0 & 0.01 & 0.03 & 0 & 0.03 & 0.11 \\
avmnist \\
push \\
enrico & 0.3 & 0.43 & 0.29 & 0.73 & 0.38 & 0.48 & 0.32 & 0.69 & 0.56 & 0.28 & 0.41 & 0.34 & & & & & 0.38 & 0.52 & 0.29 & 0.69 & \\
vqa \\
clevr \\
Average & \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{16}{c|}{\textsc{Synergy}} & \multicolumn{8}{c}{\textsc{Unique}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{Elem}} & \multicolumn{4}{c|}{\textsc{Outer}} & \multicolumn{4}{c|}{\textsc{MI}} & \multicolumn{4}{c|}{\textsc{MulT}} & \multicolumn{4}{c|}{\textsc{Lower}} & \multicolumn{4}{c}{\textsc{Rec}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
$(z_c)$ & 0.22 & 0 & 0 & 0.06 & 0.30 & 0 & 0.01 & 0.05 & 0.22 & 0.02 & 0 & 0.06 & 0.4 & 0.02 & 0 & 0.06 & 0.34 & 0 & 0.01 & 0.06 & 0.56 & 0 & 0.03 & 0.04 \\
$(z_1)$ & 0 & 0.15 & 0 & 0.05 & 0 & 0.26 & 0 & 0.05 & 0.01 & 0.14 & 0 & 0.05 & 0 & 0.48 & 0 & 0.02 & 0.01 & 0.26 & 0 & 0.05 & 0.01 & 0.55 & 0 & 0.02 \\
$(z_2)$ & 0.01 & 0 & 0.19 & 0.05 & 0 & 0 & 0.25 & 0.06 & 0.01 & 0 & 0.14 & 0.05 & 0.02 & 0 & 0.41 & 0.06 & 0 & 0 & 0.28 & 0.05 & 0.01 & 0 & 0.5 & 0.02 \\
$(z_1,z_2)$ & 0.08 & 0.01 & 0 & 0.16 & 0.10 & 0.01 & 0 & 0.19 & 0.04 & 0.01 & 0 & 0.1 & 0.16 & 0.05 & 0 & 0.29 & 0.07 & 0.02 & 0 & 0.16 & 0.15 & 0.06 & 0 & 0.35 \\
$(z_1^*,z_2^*,z_c^*)$ & 0.04 & 0 & 0 & 0.07 & 0.07 & 0.01 & 0 & 0.06 & 0.01 & 0 & 0.01 & 0.04 & 0.21 & 0.11 & 0 & 0.2 & 0.06 & 0.01 & 0 & 0.05 & 0.2 & 0.04 & 0 & 0.25 \\
$(z_1,z_2^*,z_c^*)$ & 0.05 & 0.05 & 0 & 0.07 & 0.07 & 0.03 & 0 & 0.06 & 0.03 & 0.02 & 0 & 0.06 & 0.1 & 0.29 & 0 & 0.11 & 0.05 & 0.06 & 0 & 0.06 & 0.11 & 0.24 & 0 & 0.2 \\
$(z_1,z_2,z_c^*)$ & 0.08 & 0.02 & 0 & 0.11 & 0.06 & 0 & 0.01 & 0.1 & 0.05 & 0.01 & 0 & 0.08 & 0.18 & 0.02 & 0 & 0.3 & 0.09 & 0 & 0 & 0.11 & 0.17 & 0.08 & 0 & 0.31 \\
$(z_1^*,z_2^*,z_c)$ & 0.11 & 0 & 0 & 0.09 & 0.14 & 0 & 0 & 0.06 & 0.12 & 0.01 & 0.01 & 0.06 & 0.33 & 0 & 0.03 & 0.14 & 0.15 & 0 & 0 & 0.06 & 0.35 & 0.04 & 0 & 0.19 \\
$(z_2^*,z_c^*)$ & 0.04 & 0 & 0.03 & 0.05 & 0.08 & 0.01 & 0 & 0.05 & 0.02 & 0 & 0.01 & 0.06 & 0.13 & 0 & 0.4 & 0.04 & 0.07 & 0 & 0.01 & 0.06 & 0.15 & 0 & 0.36 & 0.03 \\
$(z_2^*,z_c)$ & 0.15 & 0 & 0.03 & 0.06 & 0.18 & 0 & 0.02 & 0.06 & 0.13 & 0 & 0.01 & 0.06 & 0.36 & 0 & 0.18 & 0.04 & 0.25 & 0 & 0 & 0.06 & 0.37 & 0 & 0.18 & 0.03 \\
\hline \hline
\end{tabular}


\vspace{-4mm}
\label{tab:models}
\end{table*}

==> 02_rus/tables/maps.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\vspace{-0mm}
\caption{Results on estimating \name\ on the MAPS dataset with pairs of modalities text + apps (MAPS$_{T,A}$) and text + keystrokes (MAPS$_{T,K}$).}
\centering

\begin{tabular}{l|cccc|cccc}
\hline \hline
Dataset & \multicolumn{4}{c|}{\textsc{MAPS}$_{T,A}$} & \multicolumn{4}{c}{\textsc{MAPS}$_{T,K}$}  \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\esta & $0.09$ & $0$ & $0.09$ & $\mathbf{0.26}$ & $0.12$ & $0$ & $0.04$ & $\mathbf{0.40}$ \\
\hline \hline
\end{tabular}

\label{tab:maps}
\end{table}

\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\vspace{-0mm}
\caption{Results on estimating \name\ on model families trained on the MAPS dataset.}
\centering
\footnotesize
\vspace{-0mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{General}} & \multicolumn{10}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{EF}} & \multicolumn{5}{c|}{\textsc{Additive}} & \multicolumn{5}{c}{\textsc{Agree}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{MAPS}$_{T,A}$ & $0.61$ & $0.01$ & $\mathbf{0.08}$ & $0.02$ & $0.42$ & $0.43$ & $\mathbf{0}$ & $0.26$ & $0$ & $0.39$ & $0.45$ & $\mathbf{0}$ & $0.24$ & $0$ & $0.40$ \\
\textsc{MAPS}$_{T,K}$ & $0.16$ & $0.29$ & $0$ & $0.08$ & $0.51$ & $0.09$ & $\mathbf{0}$ & $0.18$ & $0.21$ & $0.47$ & $0.20$ & $\mathbf{0}$ & $0.24$ & $0.17$ & $0.42$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{Redundancy}} & \multicolumn{10}{c}{\textsc{Synergy}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{Align}} & \multicolumn{5}{c|}{\textsc{Elem}} & \multicolumn{5}{c}{\textsc{Tensor}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{MAPS}$_{T,A}$ & $0.69$ & $\mathbf{0}$ & $0.11$ & $0.03$ & $0.39$ & $0.42$ & $0.04$ & $0.05$ & $0.13$ & $0.41$ & $0.42$ & $0.10$ & $0.03$ & $0.11$ & $0.45$ \\
\textsc{MAPS}$_{T,K}$ & $0.41$ & $0.01$ & $0.28$ & $0.34$ & $0.33$ & $0.17$ & $0.37$ & $\mathbf{0.02}$ & $0.41$ & $0.27$ & $0.24$ & $0.15$ & $0$ & $0.32$ & $\mathbf{0.57}$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc}
\hline \hline
Category & \multicolumn{10}{c}{\textsc{Synergy}}\\
\hline
Model & \multicolumn{5}{c|}{\textsc{MI}} & \multicolumn{5}{c}{\textsc{MulT}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{MAPS}$_{T,A}$ & $\mathbf{0.28}$ & $0.12$ & $0.01$ & $\mathbf{0.21}$ & $0.47$ & $0.40$ & $0.09$ & $0$ & $0.03$ & $0.48$ \\
\textsc{MAPS}$_{T,K}$ & $0.25$ & $0.24$ & $\mathbf{0.02}$ & $\mathbf{0.40}$ & $0.36$ & $0.10$ & $0.27$ & $0$ & $0.19$ & $0.50$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc}
\hline \hline
Category & \multicolumn{10}{c}{\textsc{Unique}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{Lower}} & \multicolumn{5}{c}{\textsc{Rec}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{MAPS}$_{T,A}$ & $0.53$ & $0.04$ & $0.04$ & $0.09$ & $0.41$ & $\mathbf{0.28}$ & $0.06$ & $0.07$ & $0.10$ & $\mathbf{0.56}$ \\
\textsc{MAPS}$_{T,K}$ & $\mathbf{0.12}$ & $0.24$ & $0$ & $0.22$ & $0.51$ & $0.23$ & $0.17$ & $0$ & $0.18$ & $0.52$ \\
\hline \hline
\end{tabular}
\label{tab:maps_full}
\end{table}


==> 02_rus/tables/models_full.tex <==

\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-2mm}
\caption{Results on estimating \name\ on model families trained on synthetic datasets with controlled interactions.}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{General}} & \multicolumn{10}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{EF}} & \multicolumn{5}{c|}{\textsc{Additive}} & \multicolumn{5}{c}{\textsc{Agree}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
$(z_c)$ & $0.47$ & $0.01$ & $0.01$ & $0.04$ & $0.74$ & $0.35$ & $0.2$ & $0$ & $0.04$ & $0.71$ & $0.48$ & $0.01$ & $0.01$ & $0.06$ & $0.74$   \\
$(z_1)$ & $0$ & $0.41$ & $0$ & $0.04$ & $0.73$ & $0.02$ & $0.14$ & $0$ & $0.03$ & $0.61$ & $0.02$ & $0.15$ & $0$ & $0.04$ & $0.38$  \\
$(z_2)$ & $0.01$ & $0$ & $0.47$ & $0.04$ & $0.72$ & $0.05$ & $0$ & $0.43$ & $0.06$ & $0.72$ & $0.01$ & $0$ & $0.48$ & $0.04$ & $0.72$  \\
$(z_1,z_2)$ & $0.15$ & $0.02$ & $0$ & $0.29$ & $0.72$ & $0.15$ & $0$ & $0.2$ & $0.13$ & $0.56$ & $0.14$ & $0$ & $0.26$ & $0.09$ & $0.66$  \\
$(z_1^*,z_2^*,z_c^*)$ & $0.22$ & $0$ & $0.07$ & $0.15$ & $0.64$ & $0.31$ & $0.16$ & $0$ & $0.08$ & $0.64$ & $0.21$ & $0$ & $0.11$ & $0.15$ & $0.58$  \\
$(z_1,z_2^*,z_c^*)$ & $0.16$ & $0.15$ & $0$ & $0.15$ & $0.71$ & $0.06$ & $0$ & $0.18$ & $0.06$ & $0.6$ & $0.06$ & $0$ & $0.08$ & $0.08$ & $0.53$  \\
$(z_1,z_2,z_c^*)$ & $0.16$ & $0.05$ & $0$ & $0.25$ & $0.74$ & $0.09$ & $0$ & $0.23$ & $0.11$ & $0.52$ & $0.02$ & $0$ & $0.33$ & $0.06$ & $0.62$  \\
$(z_1^*,z_2^*,z_c)$ & $0.25$ & $0.03$ & $0$ & $0.14$ & $0.66$ & $0.39$ & $0.11$ & $0$ & $0.08$ & $0.67$ & $0.44$ & $0.04$ & $0$ & $0.09$ & $0.67$  \\
$(z_2^*,z_c^*)$ & $0.19$ & $0$ & $0.12$ & $0.06$ & $0.65$ & $0.15$ & $0$ & $0.07$ & $0.18$ & $0.61$ & $0.13$ & $0$ & $0.24$ & $0.04$ & $0.64$  \\
$(z_2^*,z_c)$ & $0.26$ & $0$ & $0.12$ & $0.05$ & $0.7$ & $0.27$ & $0$ & $0.18$ & $0.08$ & $0.71$ & $0.1$ & $0$ & $0.1$ & $0.16$ & $0.61$  \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{Redundancy}} & \multicolumn{10}{c}{\textsc{Synergy}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{Align}} & \multicolumn{5}{c|}{\textsc{Elem}} & \multicolumn{5}{c}{\textsc{Tensor}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
$(z_c)$ & $0.44$ & $0.02$ & $0$ & $0.05$ & $0.73$ & $0.27$ & $0$ & $0.01$ & $0.07$ & $0.7$ & $0.47$ & $0.01$ & $0.01$ & $0.04$ & $0.74$ \\
$(z_1)$ & $0.03$ & $0$ & $0$ & $0.05$ & $0.48$ & $0$ & $0.2$ & $0$ & $0.05$ & $0.66$ & $0$ & $0.56$ & $0$ & $0.02$ & $0.74$ \\
$(z_2)$ & $0.05$ & $0$ & $0.39$ & $0.1$ & $0.71$ & $0.01$ & $0$ & $0.2$ & $0.05$ & $0.66$ & $0.01$ & $0$ & $0.54$ & $0.02$ & $0.73$ \\
$(z_1,z_2)$ & $0.02$ & $0$ & $0.38$ & $0.08$ & $0.63$ & $0.07$ & $0.02$ & $0$ & $0.14$ & $0.66$ & $0.15$ & $0.03$ & $0$ & $0.31$ & $0.73$ \\
$(z_1^*,z_2^*,z_c^*)$ & $0.33$ & $0.06$ & $0$ & $0.15$ & $0.66$ & $0.05$ & $0$ & $0.01$ & $0.07$ & $0.56$ & $0.2$ & $0.01$ & $0.01$ & $0.21$ & $0.65$ \\
$(z_1,z_2^*,z_c^*)$ & $0.21$ & $0$ & $0.05$ & $0.14$ & $0.66$ & $0.04$ & $0.05$ & $0$ & $0.08$ & $0.61$ & $0.09$ & $0.24$ & $0$ & $0.13$ & $0.71$ \\
$(z_1,z_2,z_c^*)$ & $0.14$ & $0$ & $0.26$ & $0.04$ & $0.64$ & $0.08$ & $0.02$ & $0$ & $0.12$ & $0.66$ & $0.17$ & $0.06$ & $0$ & $0.27$ & $0.72$ \\
$(z_1^*,z_2^*,z_c)$ & $0.23$ & $0$ & $0.09$ & $0.08$ & $0.64$ & $0.1$ & $0$ & $0.01$ & $0.06$ & $0.6$ & $0.27$ & $0.05$ & $0.02$ & $0.15$ & $0.68$ \\
$(z_2^*,z_c^*)$ & $0.18$ & $0.1$ & $0$ & $0.17$ & $0.6$ & $0.04$ & $0$ & $0.03$ & $0.05$ & $0.57$ & $0.05$ & $0$ & $0.01$ & $0.06$ & $0.56$ \\
$(z_2^*,z_c)$ & $0.16$ & $0$ & $0.2$ & $0.06$ & $0.69$ & $0.15$ & $0$ & $0.03$ & $0.06$ & $0.65$ & $0.14$ & $0$ & $0.03$ & $0.05$ & $0.65$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc}
\hline \hline
Category & \multicolumn{10}{c}{\textsc{Synergy}}\\
\hline
Model & \multicolumn{5}{c|}{\textsc{MI}} & \multicolumn{5}{c}{\textsc{MulT}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
$(z_c)$ & $0.2$ & $0$ & $0.01$ & $0.05$ & $0.67$ & $0.4$ & $0.02$ & $0$ & $0.06$ & $0.73$ \\
  $(z_1)$ & $0.01$ & $0.13$ & $0$ & $0.05$ & $0.66$ & $0$ & $0.48$ & $0$ & $0.02$ & $0.73$ \\
 $(z_2)$ & $0.01$ & $0$ & $0.23$ & $0.05$ & $0.66$ & $0.02$ & $0$ & $0.42$ & $0.06$ & $0.71$ \\
 $(z_1, z_2)$ & $0.05$ & $0.04$ & $0$ & $0.12$ & $0.65$ & $0.16$ & $0.05$ & $0$ & $0.29$ & $0.72$ \\
 $(z_1^*,z_2^*,z_c^*)$ & $0.07$ & $0.01$ & $0.01$ & $0.08$ & $0.55$ & $0.21$ & $0.11$ & $0$ & $0.2$ & $0.66$ \\
 $(z_1,z_2^*,z_c^*)$ & $0.02$ & $0.01$ & $0$ & $0.06$ & $0.58$ & $0.1$ & $0.29$ & $0$ & $0.11$ & $0.7$ \\
 $(z_1,z_2,z_c^*)$ & $0.04$ & $0.01$ & $0$ & $0.08$ & $0.62$ & $0.18$ & $0.02$ & $0$ & $0.3$ & $0.72$ \\
 $(z_1^*,z_2^*,z_c)$ & $0.12$ & $0.01$ & $0.01$ & $0.06$ & $0.62$ & $0.33$ & $0$ & $0.03$ & $0.14$ & $0.68$ \\
 $(z_2^*,z_c^*)$ & $0.02$ & $0$ & $0.01$ & $0.06$ & $0.54$ & $0.13$ & $0$ & $0.39$ & $0.04$ & $0.67$ \\
 $(z_2^*,z_c)$ & $0.13$ & $0$ & $0.01$ & $0.06$ & $0.64$ & $0.36$ & $0$ & $0.18$ & $0.04$ & $0.72$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc}
\hline \hline
Category & \multicolumn{10}{c}{\textsc{Unique}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{Lower}} & \multicolumn{5}{c}{\textsc{Rec}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
$(z_c)$ & $0.53$ & $0$ & $0.01$ & $0.03$ & $0.75$ & $0.55$ & $0.02$ & $0.01$ & $0.02$ & $0.75$ \\
$(z_1)$ & $0$ & $0.56$ & $0$ & $0.02$ & $0.74$ & $0$ & $0.53$ & $0$ & $0.03$ & $0.74$ \\
$(z_2)$ & $0.01$ & $0$ & $0.54$ & $0.02$ & $0.72$ & $0.01$ & $0$ & $0.55$ & $0.02$ & $0.73$ \\
$(z_1,z_2)$ & $0.15$ & $0.03$ & $0$ & $0.32$ & $0.74$ & $0.14$ & $0.06$ & $0$ & $0.34$ & $0.74$ \\
$(z_1^*,z_2^*,z_c^*)$ & $0.21$ & $0.01$ & $0.01$ & $0.2$ & $0.65$ & $0.19$ & $0.03$ & $0$ & $0.26$ & $0.66$ \\
$(z_1,z_2^*,z_c^*)$ & $0.09$ & $0.27$ & $0$ & $0.13$ & $0.71$ & $0.08$ & $0.29$ & $0$ & $0.16$ & $0.71$ \\
$(z_1,z_2,z_c^*)$ & $0.16$ & $0.06$ & $0$ & $0.27$ & $0.73$ & $0.21$ & $0.05$ & $0$ & $0.31$ & $0.72$ \\
$(z_1^*,z_2^*,z_c)$ & $0.31$ & $0.01$ & $0.01$ & $0.16$ & $0.68$ & $0.32$ & $0$ & $0.06$ & $0.21$ & $0.68$ \\
$(z_2^*,z_c^*)$ & $0.13$ & $0$ & $0.29$ & $0.04$ & $0.64$ & $0.19$ & $0$ & $0.36$ & $0.04$ & $0.66$ \\
$(z_2^*,z_c)$ & $0.31$ & $0$ & $0.13$ & $0.04$ & $0.7$ & $0.42$ & $0$ & $0.15$ & $0.03$ & $0.72$ \\
\hline \hline
\end{tabular}


\vspace{-4mm}
\label{tab:models_full}
\end{table*}


\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-2mm}
\caption{Results on estimating \name\ on model families trained on real-world multimodal datasets.}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{General}} & \multicolumn{10}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{EF}} & \multicolumn{5}{c|}{\textsc{Additive}} & \multicolumn{5}{c}{\textsc{Agree}}\\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{UR-FUNNY a,t} & $0.02$ & $0$ & $0.02$ & $0.06$ & $0.59$ & $0.02$ & $0$ & $0.02$ & $0.15$ & $0.60$ & $0.02$ & $0$ & $0.02$ & $0.05$ & $0.59$ \\
\textsc{UR-FUNNY v,t} & $0.05$ & $0.01$ & $0$ & $0.17$ & $0.62$ & $0.11$ & $0.08$ & $0$ & $0.17$ & $0.60$ & $0.02$ & $0.04$ & $0$ & $0.24$ & $0.59$ \\
\textsc{UR-FUNNY v,a} & $0.01$ & $0.27$ & $0$ & $0.19$ & $0.59$ & $0.03$ & $0$ & $0.02$ & $0.15$ & $0.56$ & $ 0.02$ & $0$ & $0.02$ & $0.15$ & $0.53$ \\
\textsc{MOSEI a,t} & $0.16$ & $0.27$ & $0.03$ & $0$ & $0.79$ & $0.15$ & $0.19$ & $0.02$ & $0.13$ & $0.80$ & $0.14$ & $0.11$ & $0.05$ & $0.06$ & $0.80$ \\
\textsc{MOSEI v,t} & $0.01$ & $0$ & $0$ & $0$ & $0.63$ & $0.11$ & $1.21$ & $0$ & $0$ & $0.80$ & $0.1$ & $0.84$ & $0$ & $0$ & $0.80$ \\
\textsc{MOSEI v,a} & $0$ & $0$ & $0$ & $0.01$ & $0.63$ & $0.59$ & $0.62$ & $0$ & $0.12$ & $0.65$ & $0.10$ & $1.46$ & $0$ & $0.24$ & $0.61$ \\
\textsc{MUStARD a,t} & $0.06$ & $0$ & $0.03$ & $0.04$ & $0.42$ & $0.17$ & $0$ & $0.04$ & $0.33$ & $0.70$ & $0.18$ & $0$ & $0.05$ & $0.31$ & $0.68$ \\
\textsc{MUStARD v,t} & $0$ & $0$ & $0$ & $0$ & $0.57$ & $0.14$ & $0$ & $0.07$ & $0.33$ & $0.69$ & $0.19$ & $0$ & $0.07$ & $0.27$ & $0.67$ \\
\textsc{MUStARD v,a} & $0$ & $0$ & $0$ & $0$ & $0.57$ & $0.25$ & $0.12$ & $0$ & $0.15$ & $0.61$ & $0.33$ & $0.10$ & $0$ & $0.16$ & $0.58$ \\
\textsc{MIMIC} & $0.01$ & $0.27$ & $0$ & $0$ & $0.91$ & $0.01$ & $0.27$ & $0$ & $0$ & $0.92$ & $0.01$ & $0.27$ & $0$ & $0$ & $0.92$ \\
\textsc{ENRICO} & $0.71$ & $0.34$ & $0.44$ & $0.38$ & $0.50$ & $0.69$ & $0.28$ & $0.39$ & $0.35$ & $0.30$ & $0.40$ & $0.30$ & $0.52$ & $0.75$ & $0.51$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{Redundancy}} & \multicolumn{10}{c}{\textsc{Synergy}} \\
\hline
Model & \multicolumn{5}{c|}{\textsc{Align}} & \multicolumn{5}{c|}{\textsc{Elem}} & \multicolumn{5}{c}{\textsc{Tensor}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{UR-FUNNY a,t} & $0.02$ & $0$ & $0.02$ & $0.06$ & $0.58$ & $0.01$ & $0$ & $0.03$ & $0.05$ & $0.64$ & $0.01$ & $0$ & $0.02$ & $0.05$ & $0.62$ \\
\textsc{UR-FUNNY v,t} & $0.02$ & $0$ & $0.02$ & $0.15$ & $0.60$ & $0.02$ & $0.01$ & $0$ & $0.16$ & $0.61$ & $0.03$ & $0.01$ & $0$ & $0.14$ & $0.62$ \\
\textsc{UR-FUNNY v,a} & $0.12$ & $0.05$ & $0.01$ & $0.19$ & $0.53$ & $0.03$ & $0.13$ & $0$ & $0.16$ & $0.59$ & $0.02$ & $0.15$ & $0$ & $0.15$ & $0.60$ \\
\textsc{MOSEI a,t} & $0.12$ & $0.26$ & $0.14$ & $0.16$ & $0.65$ & $0.09$ & $1.07$ & $0$ & $0$ & $0.80$ & $0.18$ & $0.17$ & $0.06$ & $0$ & $0.80$ \\
\textsc{MOSEI v,t} & $0.21$ & $0.61$ & $0$ & $0.09$ & $0.65$ & $0.25$ & $0.92$ & $0$ & $0.15$ & $0.81$ & $0.12$ & $1.23$ & $0$ & $0$ & $0.81$ \\
\textsc{MOSEI v,a} & $1.15$ & $0$ & $0$ & $0.79$ & $0.40$ & $0.14$ & $1.21$ & $0$ & $0$ & $0.65$ & $0.12$ & $1.07$ & $0$ & $0$ & $0.65$ \\
\textsc{MUStARD a,t} & $0.20$ & $0$ & $0.06$ & $0.29$ & $0.70$ & $0.17$ & $0.01$ & $0.11$ & $0.23$ & $0.60$ & $0.20$ & $0$ & $0.13$ & $0.25$ & $0.59$ \\
\textsc{MUStARD v,t} & $0.16$ & $0$ & $0.08$ & $0.29$ & $0.70$ & $0.18$ & $0.01$ & $0.04$ & $0.32$ & $0.64$ & $0.18$ & $0.01$ & $0.02$ & $0.34$ & $0.59$ \\
\textsc{MUStARD v,a} & $0.27$ & $0.12$ & $0$ & $0.14$ & $0.62$ & $0.36$ & $0.07$ & $0$ & $0.16$ & $0.55$ & $0.33$ & $0.05$ & $0$ & $0.18$ & $0.60$ \\
\textsc{MIMIC} & $0.01$ & $0.28$ & $0$ & $0$ & $0.91$ & $0.04$ & $0.24$ & $0$ & $0.01$ & $0.91$ & $0$ & $0.28$ & $0$ & $0.01$ & $0.91$ \\
\textsc{ENRICO} & $0.37$ & $0.34$ & $0.57$ & $0.76$ & $0.52$ & $0.3$ & $0.43$ & $0.29$ & $0.73$ & $0.44$ & $0.38$ & $0.48$ & $0.32$ & $0.69$ & $0.50$ \\

\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|ccccc|ccccc}
\hline \hline
Category & \multicolumn{5}{c|}{\textsc{Synergy}} & \multicolumn{5}{c}{\textsc{Unique}} \\
\hline
Model  & \multicolumn{5}{c|}{\textsc{MI}} & \multicolumn{5}{c}{\textsc{Lower}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \acc & \red & \uone & \utwo & \syn & \acc \\
\hline
\textsc{UR-FUNNY a,t} & $0.01$ & $0$ & $0.03$ & $0.04$ & $0.62$ & $0.02$ & $0$ & $0.01$ & $0.14$ & $0.60$ \\
\textsc{UR-FUNNY v,t} & $0.04$ & $0.02$ & $0$ & $0.14$ & $0.64$ & $0.04$ & $0$ & $0.01$ & $0.15$ & $0.62$ \\
\textsc{UR-FUNNY v,a} & $0.02$ & $0.23$ & $0$ & $0.15$ & $0.61$ & $0.02$ & $0.15$ & $0$ & $0.19$ & $0.58$ \\
\textsc{MOSEI a,t} & $0.13$ & $0.05$ & $0.01$ & $0.19$ & $0.81$ & $0.20$ & $0.92$ & $0$ & $0.54$ & $0.79$ \\
\textsc{MOSEI v,t} & $0.11$ & $0.98$ & $0$ & $0$ & $0.80$ & $0.17$ & $1.14$ & $0$ & $0.08$ & $0.80$\\
\textsc{MOSEI v,a} & $0.12$ & $1.0$ & $0$ & $0$ & $0.65$ & $1.54$ & $0.64$ & $0$ & $0.13$ & $0.65$ \\
\textsc{MUStARD a,t} & $0.18$ & $0$ & $0.08$ & $0.29$ & $0.63$ & $0.21$ & $0$ & $0.05$ & $0.26$ & $0.59$ \\
\textsc{MUStARD v,t} & $0.20$ & $0.01$ & $0.03$ & $0.25$ & $0.63$ & $0.17$ & $0$ & $0.06$ & $0.28$ & $0.58$ \\
\textsc{MUStARD v,a} & $0.28$ & $0.04$ & $0.02$ & $0.18$ & $0.56$ & $0.24$ & $0.08$ & $0$ & $0.24$ & $0.59$ \\
\textsc{MIMIC} & $0.02$ & $0.26$ & $0$ & $0.01$ & $0.92$ & $0.01$ & $0.28$ & $0$ & $0.01$ & $0.91$ \\
\textsc{ENRICO} & $0.28$ & $0.41$ & $0.34$ & $0.48$ & $0.38$ & $0.52$ & $0.29$ & $0.69$ & $0.52$ & $0.56$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\end{table*}


==> 02_rus/tables/other_interaction.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.5pt}
\vspace{-0mm}
\caption{\small Estimating \name\ on synthetic generative model datasets. Ground truth total information is computed based on an upper bound from the best multimodal test accuracy. Both \esta\ and \estb\ measures agree with each other on relative values and are consistent with ground truth interactions. We also implement 3 other definitions: \textbf{I-min} can sometimes overestimate synergy and uniqueness; \textbf{WMS} is actually synergy minus redundancy, so can be negative and when R \& S are of equal magnitude WMS cancels out to be 0; \textbf{CI} can also be negative and sometimes incorrectly concludes highest uniqueness for S-only data.}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{$R$-only data} & \multicolumn{4}{c|}{$U_1$-only data} & \multicolumn{4}{c|}{$U_2$-only data} & \multicolumn{4}{c}{$S$-only data} \\
\hline
\name & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\textsc{I-MIN} & $0.17$ & $0.08$ & $0.07$ & $0$ & $0$ & $0.23$ & $0$ & $0.06$ & $0$ & $0$ & $0.25$ & $0.08$ & $0.07$ & $0.03$ & $0.04$ & $\mathbf{0.17}$ \\
\textsc{WMS} & $0$ & $0.20$ & $0.20$ & $-0.11$ & $0$ & $0.25$ & $0.02$ & $0.05$ & $0$ & $0.03$ & $\mathbf{0.27}$ & $0.05$ & $0$ & $0.14$ & $0.15$ & $0.07$ \\
\textsc{CI} & $\mathbf{0.34}$ & $-0.09$ & $-0.10$ & $0.17$ & $0$ & $0.23$ & $0$ & $0.06$ & $0$ & $0.01$ & $0.25$ & $0.07$ & $-0.02$ & $0.13$ & $0.14$ & $0.08$  \\
\hline
\esta & $0.16$ & $0$ & $0$ & $0.05$ & $0$ & $0.16$ & $0$ & $0.05$ & $0$ & $0$ & $0.17$ & $0.05$ & $0.07$ & $0$ & $0.01$ & $\mathbf{0.14}$ \\
\estb & $\mathbf{0.29}$ & $0.02$ & $0.02$ & $0$ & $0$ & $\mathbf{0.30}$ & $0$ & $0$ & $0$ & $0$ & $\mathbf{0.30}$ & $0$ & $0.11$ & $0.02$ & $0.02$ & $\mathbf{0.15}$ \\
\hline
Truth & $0.58$ & $0$ & $0$ & $0$ & $0$ & $0.56$ & $0$ & $0$ & $0$ & $0$ & $0.54$ & $0$ & $0$ & $0$ & $0$ & $0.56$ \\
\hline \hline
\end{tabular}

\vspace{-0mm}
\label{tab:other_interaction}
\end{table*}

==> 02_rus/tables/params.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\vspace{-0mm}
\caption{Table of hyperparameters for prediction on synthetic data.}
\centering
\footnotesize
\vspace{-2mm}

\setlength\tabcolsep{3.5pt}
\begin{tabular}{l|l|c|c}
\hline \hline
\textbf{Component} & \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\hline
\multirow{3}{*}{Encoder} & Identity & / & / \\
\cline{2-4}
& \multirow{2}{*}{Linear} & Input size & $[200, 200]$ \\ & & Hidden dim & $512$ \\
\hline 
\multirow{2}{*}{Decoder} & \multirow{2}{*}{Linear} & Input dim & $[200, 200]$ \\
& & Hidden dim & $512$ \\
\hline
\multirow{7}{*}{Fusion} & Concat & / & / \\
\cline{2-4}
& ElemMultWithLinear & \multirow{2}{*}{Output dim} & \multirow{2}{*}{$512$} \\
& MI-Matrix~\cite{Jayakumar2020Multiplicative} & & \\
\cline{2-4}
& \multirow{2}{*}{\textsc{LRTF}~\cite{liu2018efficient}} & Output dim & $512$ \\
& & rank & $32$ \\
\cline{2-4}
& \multirow{2}{*}{\textsc{MulT}~\cite{tsai2019multimodal}} & Embed dim & $512$ \\
& & Num heads & $8$ \\
\hline
\multirow{4}{*}{Classification head} & Identity & / & / \\
\cline{2-4}
& \multirow{3}{*}{2-Layer MLP} & Hidden size & $512$ \\
& & Activation & LeakyReLU($0.2$) \\
& & Dropout & 0.1 \\
\hline
\multirow{21}{*}{Training} &  & Loss & Cross Entropy \\
& \textsc{EF} \& \textsc{Additive} \& \textsc{Elem} \& \textsc{Tensor} & Batch size & $128$ \\
& \textsc{MI} \& \textsc{MulT} \& \textsc{Lower} & Num epochs & $100$ \\
& & Optimizer/Learning rate & Adam/$0.0001$ \\
\cline{2-4}
& \multirow{7}{*}{\textsc{Agree} \& \textsc{Align}} & \multirow{2}{*}{Loss} & Cross Entropy \\
& & & $+$ Agree/Align Weight \\
& & Batch size & $128$ \\
& & Num epochs & $200$ \\
& & Optimizer/Learning rate & Adam/$0.0001$ \\
& & Cross Entropy Weight & $2.0$ \\
& & Agree/Align Weight & $1.0$ \\
\cline{2-4}
& \multirow{10}{*}{\textsc{Rec}~\cite{tsai2019learning}} & \multirow{2}{*}{Loss} & Cross Entropy \\
& & & $+$ Reconstruction (MSE) \\
& & Batch size & $128$ \\
& & Num epochs & $100$\\
& & Optimizer & Adam\\
& & Learning rate & $0.0001$\\
& & Recon Loss Modality Weight & $[1,1]$\\
& & Cross Entropy Weight & $2.0$\\
& & \multirow{2}{*}{Intermediate Modules} & MLP $[512,256,256]$ \\
& & & MLP $[512,256,256]$ \\
\hline \hline
\end{tabular}
\label{tab:params_synthetic}
\end{table*}

\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\vspace{-0mm}
\caption{Table of hyperparameters for prediction on affective computing datasets.}
\centering
\footnotesize
\vspace{-2mm}

\setlength\tabcolsep{3.5pt}
\begin{tabular}{l|l|c|c}
\hline \hline
\textbf{Component} & \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\hline
\multirow{3}{*}{Encoder} & Identity & / & / \\
\cline{2-4}
& \multirow{2}{*}{GRU} & Input size & $[5, 20, 35, 74, 300, 704]$ \\ & & Hidden dim & $[32, 64, 128, 512, 1024]$ \\
\hline 
\multirow{2}{*}{Decoder} & \multirow{2}{*}{GRU} & Input size & $[5, 20, 35, 74, 300, 704]$ \\ & & Hidden dim & $[32, 64, 128, 512, 1024]$ \\
\hline
\multirow{7}{*}{Fusion} & Concat & / & / \\
\cline{2-4}
& ElemMultWithLinear & \multirow{2}{*}{Output dim} & \multirow{2}{*}{$[400, 512]$} \\
& MI-Matrix~\cite{Jayakumar2020Multiplicative} & & \\
\cline{2-4}
& Tensor Fusion~\cite{zadeh2017tensor} & Output dim & $512$  \\
\cline{2-4}
& \multirow{2}{*}{\textsc{MulT}~\cite{tsai2019multimodal}} & Embed dim & $40$ \\
& & Num heads & $8$ \\
\hline
\multirow{4}{*}{Classification head} & Identity & / & / \\
\cline{2-4}
& \multirow{3}{*}{2-Layer MLP} & Hidden size & $512$ \\
& & Activation & LeakyReLU($0.2$) \\
& & Dropout & 0.1 \\
\hline
\multirow{21}{*}{Training} &  & Loss & L1 Loss \\
& \textsc{EF} \& \textsc{Additive} \& \textsc{Elem} \& \textsc{Tensor} & Batch size & $32$ \\
& \textsc{MI} \& \textsc{MulT} \& \textsc{Lower} & Num epochs & $40$ \\
& & Optimizer/Learning rate & Adam/$0.0001$ \\
\cline{2-4}
& \multirow{7}{*}{\textsc{Agree} \& \textsc{Align}} & \multirow{2}{*}{Loss} & L1 Loss \\
& & & $+$ Agree/Align Weight \\
& & Batch size & $32$ \\
& & Num epochs & $30$ \\
& & Optimizer/Learning rate & Adam/$0.0001$ \\
& & Agree/Align Weight & $0.1$ \\
\cline{2-4}
& \multirow{10}{*}{\textsc{Rec}~\cite{tsai2019learning}} & \multirow{2}{*}{Loss} & L1 Loss \\
& & & $+$ Reconstruction (MSE) \\
& & Batch size & $128$ \\
& & Num epochs & $50$\\
& & Optimizer & Adam\\
& & Learning rate & $0.001$\\
& & Recon Loss Modality Weight & $[1,1]$\\
& & \multirow{2}{*}{Intermediate Modules} & MLP $[600,300,300]$ \\
& & & MLP $[600,300,300]$ \\
\hline \hline
\end{tabular}
\label{tab:params_affect}
\end{table*}

\begin{table*}[h]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\vspace{-0mm}
\caption{Table of hyperparameters for prediction on \textsc{ENRICO} dataset in the HCI domain.\vspace{2mm}}
\centering
\footnotesize
\vspace{-2mm}

\setlength\tabcolsep{3.5pt}
\begin{tabular}{l|c|c}
\hline \hline
 \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\hline
 Unimodal & Hidden dim & $16$ \\
 \hline
 \multirow{2}{*}{MI-Matrix~\cite{Jayakumar2020Multiplicative}} & Hidden dim & $32$ \\
 & Input dims & $16, 16$ \\
 \hline
 \multirow{2}{*}{MI} & Hidden dim & $32$ \\
 & Input dims & $16, 16$ \\
 \hline
 \multirow{3}{*}{LRTF~\cite{liu2018efficient}} & Hidden dim & $32$ \\
 & Input dims & $16, 16$ \\
 & Rank & $20$ \\
 \hline
 \multirow{7}{*}{Training} & Loss & Class-weighted Cross Entropy \\
 & Batch size & $32$ \\
 & Activation & ReLU \\
 & Dropout & $0.2$ \\
 & Optimizer & Adam \\
 & Learning Rate & $10^{-5}$ \\
 & Num epochs & $30$ \\
\hline \hline
\end{tabular}
\label{tab:params_hci}
\end{table*}

\begin{table*}[t]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Table of hyperparameters for prediction on MIMIC dataset in the healthcare domain.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | l | c | c}
\hline\hline
\textbf{Component} & \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\hline
\multirow{2}{*}{Static Encoder} & \multirow{2}{*}{2-layer MLP}
& Hidden sizes & $[10,10]$ \\
& & Activation & LeakyReLU(0.2) \\
\hline
\multirow{2}{*}{Static Decoder} & \multirow{2}{*}{2-layer MLP}
& Layer sizes & $[200,40,5]$ \\
& & Activation & LeakyReLU(0.2) \\
\hline
\multirow{1}{*}{Time Series Encoder} & \multirow{1}{*}{GRU}
& Hidden dim & $30$ \\\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{Time Series Decoder} & \multirow{1}{*}{GRU}
& Hidden dim & $30$ \\
\hline
\multirow{2}{*}{Classification Head} & \multirow{2}{*}{2-Layer MLP} & Hidden size & $40$ \\
& & Activation & LeakyReLU($0.2$) \\
\hline
\multirow{3}{*}{Fusion} & \multirow{2}{*}{LRTF~\cite{liu2018efficient}} & Output dim & $100$ \\
& & Ranks & $40$ \\
\cline{2-4}
& \multirow{1}{*}{MI-Matrix~\cite{Jayakumar2020Multiplicative}} & output dim & $100$ \\
\hline
\multirow{24}{*}{Training}
& \multirow{5}{*}{\textsc{Tensor}, \textsc{MI}} & Loss & Cross Entropy \\
& & Batch size & $40$ \\
& & Num epochs & $20$ \\
& & Optimizer & RMSprop \\
& & Learning rate & $0.001$ \\
\cline{2-4}
& \multirow{8}{*}{\textsc{Rec}~\cite{tsai2019learning}} & Loss 
& {\begin{tabular}[c]{@{}c@{}} Cross Entropy \\\ + Reconstruction(MSE) \end{tabular}} \\
& & Batch size & $40$ \\
& & Num epochs & $30$ \\
& & Optimizer & Adam \\
& & Learning Rate & $0.001$ \\
& & Recon Loss Modality Weights & $[1,1]$ \\
& & Cross Entropy Weight & $2.0$ \\
& & Intermediate Modules & {\begin{tabular}[c]{@{}c@{}} MLPs $[200,100,100]$, \\\ $[200,100,100],[400,100,100]$ \end{tabular}} \\
\cline{2-4}
\hline
\hline
\end{tabular}
\vspace{-4mm}
\label{tab:params_health}
\end{table*}

\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{6.0pt}
\vspace{-0mm}
\caption{Table of hyperparameters for prediction on MAPS.}
\centering
\footnotesize
\vspace{-2mm}

\setlength\tabcolsep{3.5pt}
\begin{tabular}{l|l|c|c}
\hline \hline
\textbf{Component} & \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\hline
\multirow{3}{*}{Encoder} & Identity & / & / \\
\cline{2-4}
& \multirow{2}{*}{Linear} & Input size & $[1000, 18, 137]$ \\ & & Hidden dim & $512$ \\
\hline 
\multirow{2}{*}{Decoder} & \multirow{2}{*}{Linear} & Input dim & $[1000, 18, 137]$ \\
& & Hidden dim & $512$ \\
\hline
\multirow{7}{*}{Fusion} & Concat & / & / \\
\cline{2-4}
& ElemMultWithLinear & \multirow{2}{*}{Output dim} & \multirow{2}{*}{$512$} \\
& MI-Matrix~\cite{Jayakumar2020Multiplicative} & & \\
\cline{2-4}
& \multirow{2}{*}{\textsc{LRTF}~\cite{liu2018efficient}} & Output dim & $512$ \\
& & rank & $32$ \\
\cline{2-4}
& \multirow{2}{*}{\textsc{MulT}~\cite{tsai2019multimodal}} & Embed dim & $512$ \\
& & Num heads & $8$ \\
\hline
\multirow{4}{*}{Classification head} & Identity & / & / \\
\cline{2-4}
& \multirow{3}{*}{2-Layer MLP} & Hidden size & $512$ \\
& & Activation & LeakyReLU($0.2$) \\
& & Dropout & 0.1 \\
\hline
\multirow{21}{*}{Training} &  & Loss & Cross Entropy \\
& \textsc{EF} \& \textsc{Additive} \& \textsc{Elem} \& \textsc{Tensor} & Batch size & $128$ \\
& \textsc{MI} \& \textsc{MulT} \& \textsc{Lower} & Num epochs & $100$ \\
& & Optimizer/Learning rate & Adam/$0.0001$ \\
\cline{2-4}
& \multirow{7}{*}{\textsc{Agree} \& \textsc{Align}} & \multirow{2}{*}{Loss} & Cross Entropy \\
& & & $+$ Agree/Align Weight \\
& & Batch size & $128$ \\
& & Num epochs & $200$ \\
& & Optimizer/Learning rate & Adam/$0.0001$ \\
& & Cross Entropy Weight & $2.0$ \\
& & Agree/Align Weight & $1.0$ \\
\cline{2-4}
& \multirow{10}{*}{\textsc{Rec}~\cite{tsai2019learning}} & \multirow{2}{*}{Loss} & Cross Entropy \\
& & & $+$ Reconstruction (MSE) \\
& & Batch size & $128$ \\
& & Num epochs & $100$\\
& & Optimizer & Adam\\
& & Learning rate & $0.0001$\\
& & Recon Loss Modality Weight & $[1,1]$\\
& & Cross Entropy Weight & $2.0$\\
& & \multirow{2}{*}{Intermediate Modules} & MLP $[512,256,256]$ \\
& & & MLP $[512,256,256]$ \\
\hline \hline
\end{tabular}
\label{tab:params_maps}
\end{table*}

\begin{table*}[t]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Table of hyperparameters for prediction on Push dataset.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | l | c | c}
\hline\hline
\textbf{Component} & \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{Pos Encoder} & \multirow{1}{*}{Linear}
& Hidden sizes & $[64, 64, 64\text{ (residual)}]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{Sensors Encoder} & \multirow{1}{*}{Linear}
& Hidden sizes & $[64, 64, 64\text{ (residual)}]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{4}{*}{Image Encoder} & \multirow{4}{*}{CNN}
& Filter sizes & $[5, 3, 3, 3, 3]$ \\
& & Num filters & $[32, 32, 32, 16, 8]$ \\
& & Filter strides & $1$ \\
& & Filter padding & $[2, 1, 1, 1, 1]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{Control Encoder} & \multirow{1}{*}{Linear}
& Hidden sizes & $[64, 64, 64\text{ (residual)}]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{4}{*}{Fusion} & \multirow{2}{*}{\shortstack[l]{\\Unimodal LSTM}}
& Hidden size & $512$ \\
& & Num layers & $2$ \\
\Xcline{2-4}{0.5\arrayrulewidth}
& \multirow{2}{*}{Late Fusion LSTM}
& Hidden size & $256$ \\
& & Num layers & $1$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{Classification Head} & \multirow{1}{*}{Linear} & \multirow{1}{*}{Hidden size} & \multirow{1}{*}{$64$} \\
\Xhline{0.5\arrayrulewidth}
\multirow{6}{*}{Training}
& & Loss & Mean Squared Error \\
& & Batch size & $32$ \\
& & Num epochs & $20$ \\
& & Activation & ReLU \\
& & Optimizer & Adam \\
& & Learning rate & $10^{-5}$ \\
\hline\hline
\end{tabular}
\vspace{-2mm}
\label{tab:robotics_params_gentle_push}
\end{table*}

\begin{table*}[t]
\fontsize{8.5}{11}\selectfont
\centering
\vspace{-2mm}
\caption{Table of hyperparameters for prediction on \textsc{AV-MNIST} dataset.\vspace{1mm}}
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l | l | c | c}
\hline\hline
\textbf{Component} & \textbf{Model} & \textbf{Parameter} & \textbf{Value} \\
\Xhline{0.5\arrayrulewidth}
\multirow{4}{*}{Image Encoder} & \multirow{4}{*}{LeNet-3}
& Filter Sizes & $[5,3,3,3]$ \\
& & Num Filters & $[6,12,24,48]$ \\
& & Filter Strides / Filter Paddings & $[1,1,1,1]$ /$[2,1,1,1]$  \\
& & Max Pooling & $[2,2,2,2]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{Image Decoder} & \multirow{3}{*}{DeLeNet-3}
& Filter Sizes & $[4,4,4,8]$ \\
& & Num Filters & $[24,12,6,3]$ \\
& & Filter Strides / Filter Paddings & $[2,2,2,4]$/$[1,1,1,1]$\\
\Xhline{0.5\arrayrulewidth}
\multirow{4}{*}{Audio Encoder} & \multirow{4}{*}{LeNet-5}
& Filter Sizes & $[5,3,3,3,3,3]$ \\
& & Num Filters & $[6,12,24,48,96,192]$ \\
& & Filter Strides / Filter Paddings & $[1,1,1,1,1,1]$/$[2,1,1,1,1,1]$ \\
& & Max Pooling & $[2,2,2,2,2,2]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{Audio Decoder} & \multirow{3}{*}{DeLeNet-5}
& Filter Sizes & $[4,4,4,4,4,8]$ \\
& & Num Filters & $[96,48,24,12,6,3]$ \\
& & Filter Strides / Filter Paddings & $[2,2,2,2,2,4]$/$[1,1,1,1,1,1]$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{Classification Head} & \multirow{2}{*}{2-Layer MLP} & Hidden size & $100$ \\
& & Activation & LeakyReLU($0.2$) \\
\Xhline{0.5\arrayrulewidth}
\multirow{4}{*}{Training}
& \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Unimodal, LF\end{tabular}} & Loss & Cross Entropy \\
& & Batch size & $40$ \\
& & Num epochs & $25$ \\
& & Optimizer/Learning rate/weight decay & SGD/$0.05$/$0.0001$ \\
\hline\hline
\end{tabular}
\vspace{-4mm}
\label{multimedia_params1}
\end{table*}

==> 02_rus/tables/robotics.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\vspace{-0mm}
\caption{Results on estimating \name\ on robotic perception task.}
\centering

\begin{tabular}{l|cccc}
\hline \hline
Task & \multicolumn{4}{c}{\textsc{Push i,c}} \\
\hline
Measure & \red & \uone & \utwo & \syn \\
\hline
\esta & $0.24$ & $0.03$ & $0.06$ & $0.04$ \\
\estb & $0.75$ & $1.79$ & $0.03$ & $0.08$ \\
\hline \hline
\end{tabular}

\label{tab:robotics}
\end{table}


==> 02_rus/tables/setup.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\vspace{1mm}
\caption{Collection of datasets used for our study of multimodal fusion interactions covering diverse modalities, tasks, and research areas in multimedia and affective computing.}
\centering
\vspace{1mm}
\begin{tabular}{l|ccccc}
\hline \hline
Datasets & Modalities & Size & Prediction task & Research Area \\
\hline
\textsc{MUStARD}~\cite{castro2019towards} & $\{ \textrm{text}, \textrm{video}, \textrm{audio} \}$ & $690$ & sarcasm & Affective Computing \\
\textsc{UR-FUNNY}~\cite{hasan2019ur} & $\{ \textrm{text}, \textrm{video}, \textrm{audio} \}$ & $16,514$ & humor & Affective Computing \\
\textsc{MOSEI}~\cite{zadeh2018multimodal} & $\{ \textrm{text}, \textrm{video}, \textrm{audio} \}$ & $22,777$ & sentiment, emotions & Affective Computing \\
\textsc{CLEVR}~\cite{johnson2017clevr} & $\{ \textrm{image}, \textrm{question} \}$ & $853,554$ & QA & Multimedia \\
\textsc{VQA 2.0}~\cite{goyal2017making} & $\{ \textrm{image}, \textrm{question} \}$ & $1,100,000$ & QA & Multimedia \\
\hline \hline
\end{tabular}

\vspace{-2mm}
\label{tab:setup}
\end{table*}

==> 02_rus/tables/tcga.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\vspace{-0mm}
\caption{Results on estimating \name\ across the TCGA-GBMLGG and TCGA-PAAD datasets. $U_1, U_2$ correspond to pathology and genomics respectively.}
\centering

\begin{tabular}{l|cccc|cccc}
\hline \hline
Dataset & \multicolumn{4}{c|}{\textsc{TCGA-LGG}} & \multicolumn{4}{c}{\textsc{TCGA-PAAD}}  \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
%\esta & 0.01 & 0 & 0.11 & 0.04 & 0.02 & 0.19 & 0.09 & 0.18 \\
\esta & $0$ & $0.02$ & $\mathbf{0.06}$ & $0.02$ & $0$ & $0.06$ & $\mathbf{0.08}$ & $\mathbf{0.15}$ \\
\hline \hline
\end{tabular}

\label{tab:tcga}
\end{table}


==> 03_factorcl/tables/additional.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2pt}
\caption{Additional experiments on CIFAR10~\cite{Krizhevsky} and MNIST~\cite{deng2012mnist} datasets using our \names\ objectives on image classification.}
\centering
\begin{tabular}{l|c c c}
\hline \hline
Task & \textsc{CIFAR10} & \textsc{MNIST}\\
\hline
SimCLR~\cite{chen2020simple} & 87.0\% & 98.84\%\\
SupCon~\cite{khosla2020supervised} & 92.7\% & 99.38\%\\
\names-SUP & 91.3\% & 99.21\%\\
\hline \hline
\end{tabular}
\label{tab:additional}
\end{table*}

==> 03_factorcl/tables/augs.tex <==
\begin{table*}[t]
\centering
\fontsize{8}{11}\selectfont
\setlength\tabcolsep{2pt}
\vspace{-0mm}
\caption{More examples of optimal single-view and multi-view augmentations.}
\centering

\begin{tabular}{l c c c c c c c }
\hline 
& & & & Standard Aug & \textbf{Unique Aug} \\
Dataset & $X_1$ & $X_2$ &$X_1'$ & $X_2'$ & $X_2''$ \\
\hline
Cartoon & Caption & Image & Word Masking & Crop + Flip + Resize & Flip + Resize \\
MIMIC & Signals & Tables & Time Warping & CutMix \cite{yun2019cutmix} on All Features & CutMix on Nonclinical Features \\
MOSEI & Transcripts & Video+Audio & Word Masking & Noise Injection on Any Frames & Noise Injection on Silent Frames\\
UR-FUNNY & Transcripts & Video+Audio & Word Masking & Noise Injection on Any Frames & Noise Injection on Silent Frames \\
MUsTARD & Transcripts & Video+Audio & Word Masking & Noise Injection on Any Frames & Noise Injection on Silent Frames \\
\hline \hline
\end{tabular}

\vspace{-0mm}
\label{tab:augs}
\end{table*}

==> 03_factorcl/tables/infomin_probe.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{4pt}
\caption{We probe whether the InfoMin assumption from Tian et al., $I(Z_1; Y | X_2) = 0$ and $I(Z_2; Y | X_1) = 0$, is reasonable for Theorem 1. Compared to the shared information $I(X_1; X_2)$, $I(Z_1; Y | X_2)$ is much smaller and closer to zero, indicating that the InfoMin assumption is reasonable, and Theorem 1 holds in practice.}
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline \hline
$I(X_1, Y;X_2)$ & $I(X_1; X_2)$ & $I(Z_1; Y | X_2)$ & $I(X_2, Y;X_1)$ & $I(X_2; X_1)$ & $I(Z_2; Y | X_1)$ \\
\hline
12.69 & 12.29 & 0.40 & 11.31 & 10.92 & 0.38 \\
\hline \hline
\end{tabular}
\label{tab:probing_mi_conditional}
\end{table*}

==> 04_multiviz/alg.tex <==
\begin{figure}
    \begin{minipage}{\linewidth}
    \vspace{-4mm}
    \begin{algorithm}[H]
    \caption{Visualizing and understanding multimodal models using \name.}
    \begin{algorithmic}
    \State \textbf{Given:} Dataset $\mathcal{D} = \{ (\mathbf{x}_1, \mathbf{x}_2, y)_{i=1}^n \} = \{ ( x_1^{(1)}, ..., x_2^{(1)}, ..., y )_{i=1}^n \}$ and trained model $f_\theta$.
    \State \textbf{Given:} Unimodal and cross-modal visualization subroutines $\textsc{Uni}(f_\theta, y, \mathbf{x})$, $\textsc{CM}(f_\theta, y, x_1, \mathbf{x}_2)$.
    \State Obtain deep features $M_z = f_{\theta} (\mathbf{x}_1, \mathbf{x}_2)$ for datapoint of interest.
    \State Fit sparse linear model: $f_{\theta \textrm{sparse}} = M_z^\top \hat{\beta}$ by solving equation~\eqref{sparse_eqn}.
    \State Obtain predictions $\hat{y} = f_{\theta \textrm{sparse}} (\mathbf{x}_1, \mathbf{x}_2)$ and ranked features $z_{\textrm{top}}$ with largest coefficients.
    \State Visualize overall unimodal importance wrt $\hat{y}$: $U_1 = \textsc{Uni}(f_\theta, \hat{y}, \mathbf{x}_1), U_2 = \textsc{Uni}(f_\theta, \hat{y}, \mathbf{x}_2)$.
    \State Visualize overall cross-modal interactions wrt $\hat{y}$: $C = \textsc{CM}(f_\theta, \hat{y}, x_1, \mathbf{x}_2)$, $\textsc{CM}(f_\theta, \hat{y}, x_2, \mathbf{x}_1)$.
    \For{each top feature $z$ in $z_{\textrm{top}}$}
        \State \texttt{\# local analysis for original datapoint}
        \State Visualize unimodal and cross-modal interactions of original datapoint wrt $z$.
        \State \texttt{\# global analysis across similar datapoints}
        \State Obtain top $k$ datapoints that also maximally activate $z$.
        \For{each new top $k$ datapoint $(\mathbf{x}_1, \mathbf{x}_2, y)$}
            \State Visualize unimodal and cross-modal interactions of new datapoint wrt $z$.
        \EndFor
    \EndFor
    \end{algorithmic}
    \label{algotex}
    \end{algorithm}
    \end{minipage}
    \vspace{-2mm}
\end{figure}

==> 04_multiviz/tables/debugging.tex <==
\begin{table*}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-0mm}
\caption{\textbf{Model debugging}: we task $3$ human users to use \name\ visualizations and highlight the bugs that a model exhibits (see Figure~\ref{fig:human2}), and find $2$ penultimate-layer neurons which highlighted the model's failure to identify color. The model has an accuracy of only $5.5\%$ amongst all blue-related points (i.e., either have blue as correct answer or predicted answer), and these failures account for $8.8\%$ of all model errors. By providing the model with $500$ additional datapoints asking specifically about color (in an active learning setup), we improve the model, especially on the targeted points.}
\centering
\footnotesize
\vspace{-0mm}
\begin{tabular}{l|cccccccc}
\hline \hline
Research area & \multicolumn{2}{c}{QA} \\
Dataset & \multicolumn{2}{c}{\textsc{VQA 2.0}~\citep{goyal2017making}} \\
Model & \multicolumn{2}{c}{\textsc{LXMERT}~\citep{lxmert}} \\
\hline
Metric & Targeted accuracy $\Delta$ & Overall accuracy $\Delta$ \\
\hline
% \multirow{3}{*}{Fusion} & \multirow{3}{*}{\textsc{MM-IMDb}~\citep{arevalo2017gated}} & \multirow{3}{*}{\textsc{LF}~\citep{baltruvsaitis2018multimodal}} & Random & \\
% & & & Uncertainty & \\
% & & & \name\ & \\ \hline
% \multirow{3}{*}{Retrieval} & \multirow{3}{*}{\textsc{Flickr-30k}~\citep{plummer2015flickr30k}} & % \multirow{3}{*}{\textsc{ViLBERT}~\citep{lu2019vilbert}} & Random & \\
% & & & Uncertainty & \\
% & & & \name\ & \\ \hline
Random & $+1.4 \pm 0.3$ & $+0.3 \pm 0.1$ \\
Uncertainty~\citep{lewis1994heterogeneous} & $+0.0 \pm 0.0$ & $+0.1 \pm 0.0$ \\
\name\ no color & $+2.5 \pm 1.3$ & $+0.1 \pm 0.0$ \\
\name\ 1 color & $+27.5 \pm 1.9$ & $+1.0 \pm 0.1$ \\
\name\ 2 color & $\mathbf{+30.5 \pm 4.9}$ & $\mathbf{+1.2 \pm 0.2}$ \\
\hline \hline
\end{tabular}
\vspace{-4mm}
\label{tab:debugging}
\end{table*}

==> 04_multiviz/tables/local_app.tex <==
\begin{table*}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{1.5pt}
\vspace{-0mm}
\caption{Local faithfulness evaluations on visualizing cross-modal interactions. We study the correlation between model performance and what cross-modal interactions are picked up by the model. Across 2 models on CLEVR, we find that the ability to capture cross-modal alignment, as judged by \name, correlates strongly with final task performance.}
\centering
\footnotesize
\vspace{-0mm}
\begin{tabular}{l|cc|ccc}
\hline\hline
Method & Dataset & Model & \begin{tabular}[c]{@{}c@{}}Model\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Top 1 alignment\\accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Top 2 alignment\\accuracy\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Second Order\\ Gradient\end{tabular}} & \multirow{2}{*}{CLEVR} & MDETR~\citep{kamath2021mdetr} & $99.5\%$ & $55.8\%$ & $80.7\%$ \\
& & CNN+LSTM+SA~\citep{johnson2017clevr} & $68.5\%$ & $21.2\%$ & $32.7\%$ \\
\hline\hline
\end{tabular}
\vspace{-4mm}
\label{tab:local_app}
\end{table*}

==> 04_multiviz/tables/local_error.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-0mm}
\caption{Humans are able to consistently perform error analysis on trained models. TODO}
\centering
\footnotesize
\vspace{-0mm}
\begin{tabular}{l|cccccccc}
\hline \hline
\multicolumn{1}{l|}{Level} & Dataset & Model & Method & Confidence & Agreement ($\alpha$)~\citep{krippendorff2011computing} \\ \hline
\multirow{3}{*}{\makecell[l]{Error\\analysis}} & \multirow{3}{*}{\textsc{VQA 2.0}~\citep{goyal2017making}} & \multirow{3}{*}{\textsc{LXMERT}~\citep{lxmert}} & ?? \\
& & & ?? \\
& & & ?? \\
\hline \hline
\end{tabular}
\vspace{-2mm}
\label{tab:local_error}
\end{table*}

==> 04_multiviz/tables/overall.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-0mm}
\caption{We scaffold the problem of interpreting multimodal models into the following stages for which algorithm design and analysis can occur. For each step, \name\ includes existing and newly proposed approaches for visualizing models across modalities and tasks.}
\centering
\footnotesize
\vspace{-0mm}
\begin{tabular}{l|cccccccc}
\hline \hline
\multicolumn{1}{l|}{Level} & Methods \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{Unimodal importance} & Gradient~\citep{simonyan2013deep,baehrens2010explain,erhan2009visualizing},\\ & LIME~\citep{han2020explaining,lime,yosinski2015understanding},\\ & SHAP~\citep{merrick2020explanation,rodriguez2020interpretation} \\ \hline
\multirow{2}{*}{Cross-modal interactions} & Cross-modal $\{$Gradient, LIME, SHAP$\}$ (new),\\
& EMAP~\citep{hessel2020does}, DIME~\citep{lyu2022dime} \\ \hline
\multirow{1}{*}{Multimodal representation} & Local \& global analysis (new) \\ \hline
\multirow{1}{*}{Multimodal prediction} & Sparse linear model (new) \\ \hline \hline
% \multirow{2}{*}{Intervention} & Natural imperfections & Modality-specific \& multimodal noises \\
% & Targeted interventions & Causal \& counterfactual interventions \\
\end{tabular}
\vspace{-2mm}
\label{tab:overall}
\end{table*}

==> 05_bounds/figures/masking.tex <==
\begin{wrapfigure}{R}{0.6\textwidth}
    \vspace{-4mm}
    \begin{minipage}{0.6\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/merlot_fig.pdf}
    \vspace{-6mm}
    \caption{Masked predictions do not always agree across modalities, as shown in this example from the Social-IQ dataset. Adding a slack term enabling pre-training with modality disagreement yields strong performance improvement over baselines.}
    \label{fig:masking}
    \end{minipage}
\vspace{-2mm}
\end{wrapfigure}

==> 05_bounds/figures/plots.tex <==
\begin{figure*}[t]
\centering
\vspace{-6mm}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/best_fit/lower_bound_diff.pdf}
  \caption{$S$ vs $\lowa$}
  \label{fig:lower_bound1}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/best_fit/lower_bound_R.pdf}
  \caption{$S$ vs $\lowb$}
  \label{fig:lower_bound2}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/best_fit/upper_bound.pdf}
  \caption{$S$ vs $\high$}
  \label{fig:upper_bound}
\end{subfigure}%
\vspace{-1mm}
\caption{Plots of actual synergy against our estimated (a) lower bound on synergy $\lowa$, (b) lower bound on synergy $\lowa$, and (c) upper bound $\high$. The bounds closely track true synergy, which we show via three lines of best fit that almost exactly track true synergy: $y=1.095x$, $y=1.098x$, and $y=x-0.2$.}
\vspace{-4mm}
\label{fig:plots}
\end{figure*}

==> 05_bounds/tables/all_bounds.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{1.0pt}
\vspace{-4mm}
\caption{We show the full list of computed lower and upper bounds on $S$ without labeled multimodal data and compare them to the true $S$ assuming knowledge of the full joint distribution $p$: the bounds track $S$ well on \textsc{MUStARD} and \textsc{MIMIC}, and also show general trends on the other datasets except \textsc{ENRICO} where estimating synergy is difficult. V = video, T = text, A = audio modalities.}
\vspace{1mm}
\centering
\footnotesize
\begin{tabular}{l|cccccccccccccccccccc}

\hline \hline
& \textsc{MOSEI$_\text{V+T}$} & \textsc{MOSEI$_\text{V+A}$} & \textsc{MOSEI$_\text{A+T}$} & \textsc{UR-FUNNY$_\text{V+T}$} & \textsc{UR-FUNNY$_\text{V+A}$} & \textsc{UR-FUNNY$_\text{A+T}$}  \\
\hline
$\high$ & $0.96$ & $0.98$ & $0.97$ & $0.96$ & $0.96$ & $0.99$ \\
$S$ & $0.04$ & $0.03$ & $0.03$ & $0.21$ & $0.24$ & $0.08$ \\
$\lowa$ & $0.01$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\
$\lowb$ & $0.01$ & $0.01$ & $0.0$ & $0.0$ & $0.0$ & $0.01$ \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccccccccccccccccccc}
\hline\hline
& \textsc{MOSI$_\text{V,T}$} & \textsc{MOSI$_\text{V,A}$} & \textsc{MOSI$_\text{A,T}$} & \textsc{MUStARD$_\text{V,T}$} & \textsc{MUStARD$_\text{V,A}$} & \textsc{MUStARD$_\text{A,T}$} & \textsc{MIMIC} & \textsc{ENRICO} \\
\hline
$\high$ & $0.92$ & $0.92$ & $0.93$ & $0.79$ & $0.78$ & $0.79$ & $0.41$ & $2.09$ \\
$S$ & $0.31$ & $0.28$ & $0.14$ & $0.49$ & $0.31$ & $0.51$ & $0.02$ & $1.02$ \\
$\lowa$ & $0.01$ & $0.01$ & $0.0$ & $0.04$ & $0.01$ & $0.06$ & $0.0$ & $0.01$ \\
$\lowb$ & $0.03$ & $0.03$ & $0.02$ & $0.07$ & $0.06$ & $0.11$ & $-0.12$ & $-0.55$ \\
\hline \hline
\end{tabular}

\vspace{-2mm}
\label{tab:s_app}
\end{table}

==> 05_bounds/tables/bit_example.tex <==
\begin{wraptable}{r}{3.5cm}
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.0pt}
\vspace{-4mm}
\caption{small example. TODO find best one}
\centering
\footnotesize
\begin{tabular}{ccc|c}
\hline \hline
$x_1$ & $x_2$ & $y$ & $p$ \\
\hline
$0$ & $0$ & $0$ & $0.231$ \\
$0$ & $0$ & $1$ & $0.009$ \\
$0$ & $1$ & $0$ & $0.071$ \\
$0$ & $1$ & $1$ & $0.007$ \\
$1$ & $0$ & $0$ & $0.018$ \\
$1$ & $0$ & $1$ & $0.424$ \\
$1$ & $1$ & $0$ & $0.224$ \\
$1$ & $1$ & $1$ & $0.016$ \\
\hline \hline
\end{tabular}

\vspace{-4mm}
\label{tab:bit_example}
\end{wraptable}


==> 05_bounds/tables/fusion.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2pt}
\vspace{-0mm}
\caption{Estimated bounds on real-world MultiBench~\citep{liang2021multibench} datasets.}
\centering
\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{MIMIC}} & \multicolumn{4}{c|}{\textsc{AV-MNIST}} & \multicolumn{4}{c|}{\textsc{ENRICO}} & \multicolumn{4}{c|}{\textsc{MOSEI}} & \multicolumn{4}{c|}{\textsc{UR-FUNNY}} & \multicolumn{4}{c}{\textsc{MUStARD}}\\
\hline
Measure & $R$ & $U_1$ & $U_2$ & $S$ & $R$ & $U_1$ & $U_2$ & $S$ & $R$ & $U_1$ & $U_2$ & $S$ & $R$ & $U_1$ & $U_2$ & $S$ & $R$ & $U_1$ & $U_2$ & $S$ & $R$ & $U_1$ & $U_2$ & $S$\\
\hline
Value & $0.05$ & $0.17$ & 0 & 0.01 & 0.10 & 0.97 & 0.03 &0.08 &0.73 &0.38 &0.53 &0.34 &0.26 &0.49 &0.03 &0.04 &0.03 &0.01 &0.04 &0.08 &0.14 &0.01 &0.01 &0.30\\
\hline \hline
\end{tabular}

\vspace{-0mm}
\label{tab:fusion}
\end{table*}

==> 05_bounds/tables/masking.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3pt}
\vspace{-4mm}
\caption{Allowing for disagreement during self-supervised masked pre-training yields performance improvements on these datasets. Over $10$ runs, improvements that are statistically significant are shown in bold ($p<0.05$).}
\begin{tabular}{l|cccccccccccc}
\hline \hline
& \textsc{Social-IQ} & \textsc{UR-FUNNY} & \textsc{MUStARD} & \textsc{Cartoon} & \textsc{TVQA} \\
\hline
FLAVA, MERLOT Reserve & $70.6\pm 0.6$ & $80.0\pm 0.7$ & $77.4\pm 0.8$ & $38.6\pm0.6$ & $82.0$\\
+ disagreement & $\mathbf{71.1\pm0.5}$ & $\mathbf{80.7\pm 0.5}$ & $\mathbf{78.1\pm1.1}$ & $39.3\pm0.5$ & $83.0$\\
\hline \hline
\end{tabular}
\label{tab:masking}
\vspace{-2mm}
\end{table*}

==> 05_bounds/tables/others.tex <==
\newcommand{\red}{$R$}
\newcommand{\uone}{$U_1$}
\newcommand{\utwo}{$U_2$}
\newcommand{\syn}{$S$}

\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{2.5pt}
\vspace{-0mm}
\caption{\color{red} Estimating multimodal interactions on synthetic generative model datasets. Ground truth total information is computed based on an upper bound from the best multimodal test accuracy. Our estimated interactions are consistent with ground truth interactions. We also implement 3 other definitions: \textbf{I-min} can sometimes overestimate synergy and uniqueness; \textbf{WMS} is actually synergy minus redundancy, so can be negative and when $R$ \& $S$ are of equal magnitude WMS cancels out to be 0; \textbf{CI} can also be negative and sometimes incorrectly concludes highest uniqueness for S-only data.}
\centering
\footnotesize
\vspace{-2mm}

{\color{red}\begin{tabular}{l|cccc|cccc|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{$R$-only data} & \multicolumn{4}{c|}{$U_1$-only data} & \multicolumn{4}{c|}{$U_2$-only data} & \multicolumn{4}{c}{$S$-only data} \\
\hline
Interaction & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\textsc{I-MIN} & $0.17$ & $0.08$ & $0.07$ & $0$ & $0$ & $0.23$ & $0$ & $0.06$ & $0$ & $0$ & $0.25$ & $0.08$ & $0.07$ & $0.03$ & $0.04$ & $\mathbf{0.17}$ \\
\textsc{WMS} & $0$ & $0.20$ & $0.20$ & $-0.11$ & $0$ & $0.25$ & $0.02$ & $0.05$ & $0$ & $0.03$ & $\mathbf{0.27}$ & $0.05$ & $0$ & $0.14$ & $0.15$ & $0.07$ \\
\textsc{CI} & $\mathbf{0.34}$ & $-0.09$ & $-0.10$ & $0.17$ & $0$ & $0.23$ & $0$ & $0.06$ & $0$ & $0.01$ & $0.25$ & $0.07$ & $-0.02$ & $0.13$ & $0.14$ & $0.08$  \\
\hline
\textbf{Ours} & $0.16$ & $0$ & $0$ & $0.05$ & $0$ & $0.16$ & $0$ & $0.05$ & $0$ & $0$ & $0.17$ & $0.05$ & $0.07$ & $0$ & $0.01$ & $\mathbf{0.14}$ \\
\hline
Truth & $0.58$ & $0$ & $0$ & $0$ & $0$ & $0.56$ & $0$ & $0$ & $0$ & $0$ & $0.54$ & $0$ & $0$ & $0$ & $0$ & $0.56$ \\
\hline \hline
\end{tabular}
}

\vspace{-0mm}
\label{tab:other_interaction}
\end{table*}

==> 05_bounds/tables/perf_app.tex <==
\begin{table}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{1.0pt}
\vspace{-4mm}
\caption{Full list of best unimodal performance $P_\textrm{acc}(f_i)$, best simple fusion $P_\textrm{acc}(f_{M\textrm{simple}})$, and best complex fusion $P_\textrm{acc}(f_{M\textrm{complex}})$ as obtained from the most recent state-of-the-art models. We also include our estimated bounds $(\underline{P}_\textrm{acc}(f_M^*), \overline{P}_\textrm{acc}(f_M^*))$ on optimal multimodal performance.}
\vspace{1mm}
\centering
\footnotesize

\begin{tabular}{l|ccccccc}
\hline \hline
& \textsc{MOSEI} & \textsc{UR-FUNNY} & \textsc{MOSI} \\
\hline
$\overline{P}_\textrm{acc}(f_M^*)$ & $1.07$ & $1.21$ & $1.29$ \\
$P_\textrm{acc}(f_{M\textrm{complex}})$ & $0.88$ \citep{hu-etal-2022-unimse} & $0.77$ \citep{Hasan_Lee_Rahman_Zadeh_Mihalcea_Morency_Hoque_2021} & $0.86$ \citep{hu-etal-2022-unimse} \\
$P_\textrm{acc}(f_{M\textrm{simple}})$ & $0.85$ \citep{rahman-etal-2020-integrating} & $0.76$ \citep{Hasan_Lee_Rahman_Zadeh_Mihalcea_Morency_Hoque_2021} & $0.84$ \citep{rahman-etal-2020-integrating} \\
$P_\textrm{acc}(f_i)$ & $0.82$ \citep{delbrouck-etal-2020-transformer} & $0.74$ \citep{Hasan_Lee_Rahman_Zadeh_Mihalcea_Morency_Hoque_2021} & $0.83$ \citep{10.1145/3394171.3413690} \\
$\underline{P}_\textrm{acc}(f_M^*)$ & $0.52$ & $0.58$ & $0.62$ \\
\hline \hline
\end{tabular}

\vspace{2mm}

\begin{tabular}{l|ccccccc}
\hline \hline
& \textsc{MUStARD} & \textsc{MIMIC} & \textsc{ENRICO} \\
\hline
$\overline{P}_\textrm{acc}(f_M^*)$ & $1.63$ & $1.27$ & $0.88$\\
$P_\textrm{acc}(f_{M\textrm{complex}})$ & $0.79$ \citep{Hasan_Lee_Rahman_Zadeh_Mihalcea_Morency_Hoque_2021} & $0.92$ \citep{liang2021multibench} & $0.51$ \citep{liang2021multibench} \\
$P_\textrm{acc}(f_{M\textrm{simple}})$ & $0.74$ \citep{Pramanick2021MultimodalLU} & $0.92$ \citep{liang2021multibench} & $0.49$ \citep{liang2021multibench} \\
$P_\textrm{acc}(f_i)$ & $0.74$ \citep{Hasan_Lee_Rahman_Zadeh_Mihalcea_Morency_Hoque_2021} & $0.92$ \citep{liang2021multibench} & $0.47$ \citep{liang2021multibench} \\
$\underline{P}_\textrm{acc}(f_M^*)$ & $0.78$ & $0.76$ & $0.48$ \\
\hline \hline
\end{tabular}

\vspace{-2mm}
\label{tab:acc_app}
\end{table}

==> 06_multibench/data/models.tex <==
\begin{table*}[]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\caption{\codes\ provides a standardized implementation of the following multimodal methods to enable accessibility for new researchers and reproducibility of results. These approaches span advances in data processing, fusion paradigms, optimization objectives, and training procedures. We choose these approaches since they offer complementary perspectives towards tacking the fundamental challenges in multimodal fusion: (1) aligning signals across modalities at the right granularity, (2) learning complementary information across aligned signals, and (3) maintaining robustness in the presence of noisy and missing modalities.}
\centering
\footnotesize
\vspace{-0mm}

\begin{tabular}{c|c|c|c|c}
\hline \hline
Category & Method & Alignment & Complementarity & Robustness \\
\hline
\multirow{1}{*}{Data} & \textsc{WordAlign}~\cite{chen2017multimodal} & \textcolor{gg}\cmark & \textcolor{rr}\xmark & \textcolor{rr}\xmark \\
\hline
\multirow{6}{*}{Model} & \textsc{EF}, \textsc{LF}~\cite{baltruvsaitis2018multimodal} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{TF}~\citep{zadeh2017tensor}, \textsc{LRTF}~\citep{liu2018efficient} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{MI-Matrix}, \textsc{MI-Vector}, \textsc{MI-Scalar}~\citep{Jayakumar2020Multiplicative} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{NL Gate}~\cite{wang2020makes} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{MulT}~\citep{tsai2019multimodal} & \textcolor{gg}\cmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{MFAS}~\citep{perez2019mfas} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
\hline
\multirow{5}{*}{Objective} & \textsc{CCA}~\citep{andrew2013deep} & \textcolor{gg}\cmark & \textcolor{rr}\xmark & \textcolor{rr}\xmark \\
& \textsc{ReFNet}~\cite{sankaran2021multimodal} & \textcolor{gg}\cmark & \textcolor{rr}\xmark & \textcolor{rr}\xmark \\
& \textsc{MFM}~\cite{tsai2019learning} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{MVAE}~\citep{wu2018multimodal} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark \\
& \textsc{MCTN}~\citep{pham2019found} & \textcolor{rr}\xmark & \textcolor{rr}\xmark & \textcolor{gg}\cmark \\
\hline
\multirow{2}{*}{Training} & \textsc{GradBlend}~\citep{wang2020makes} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{gg}\cmark \\
& \textsc{RMFE}~\cite{gat2020removing} & \textcolor{rr}\xmark & \textcolor{gg}\cmark & \textcolor{gg}\cmark \\
\hline \hline
\end{tabular}

\vspace{-4mm}
\label{multibench:data:models}
\end{table*}

==> 07_rmfn/figures/blocks.tex <==
\begin{figure}[t!]
\centering{
\includegraphics[width=\linewidth]{07_rmfn/figures/blocks_fig.pdf}}
    \caption{A close-up of the \texttt{HIGHLIGHT} and \texttt{FUSE} operations in the \ourl. $\mathbb{A}$ is the the memory of the \texttt{HIGHLIGHT} module. $\mathbb{S}$ is the memory of the \texttt{FUSE} module. The \texttt{HIGHLIGHT} and \texttt{FUSE} operations are both dependent on representations from previous stages that are stored in $\mathbb{A}$ and $\mathbb{S}$ respectively.}
    \label{fig:blocks}
\end{figure}

==> 08_highmmt/figures/compare.tex <==
\begin{figure*}[tbp]
\centering
\vspace{-0mm}
\includegraphics[width=\linewidth]{08_highmmt/figures/compare_fig.pdf}
\caption{In contrast to current work in unified unimodal encoders~\citep{jaegle2021perceiver,kaiser2017one,li2021towards,likhosherstov2022polyvit} and multimodal multitask learning~\citep{hu2021transformer,lu2019vilbert,Su2020VLBERT,cho2021vlt5,akbari2021vatt,singh2021flava}, we aim to design a general-purpose model for high-modality and partially-observable scenarios, which presents two main technical challenges: (1) \textit{scalability}, since adding new parameters for every new modality/task becomes prohibitively expensive, and (2) \textit{partial observability}, since each task is defined only over a small subset of all modalities we are interested in modeling.}
\label{fig:compare}
\vspace{-2mm}
\end{figure*}

==> 08_highmmt/figures/fewshot.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{08_highmmt/figures/fewshot_fig.pdf}
\caption{\textbf{Few-shot results} on new modalities and tasks. Multimodal multitask training using \names\ learns more generalizable representations which improves performance across all ranges of data. The $x$-axis shows the percentage of labeled data used during training.}
\label{fig:fewshot}
\vspace{-2mm}
\end{figure*}

==> 08_highmmt/tables/multitask.tex <==
\begin{table*}[]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{4.0pt}
\caption{\names\ achieves strong performance on overall performance and efficiency, sometimes even beating (shown in \textbf{bold}) the task-specific state-of-the-art, especially on the relatively understudied modalities (time-series, robotics sensors, and sets) from the robotics (\textsc{Push}, \textsc{V\&T}) and HCI (\textsc{ENRICO}) research areas. MultiBench range captures the min and max (SOTA) performance and parameters of more than $20$ recent multimodal models implemented in~\citet{liang2021multibench}.} 
\centering
\footnotesize
\vspace{1mm}

\begin{tabular}{l|cc|c}
\Xhline{3\arrayrulewidth}
Small setting & \textsc{Push} $\downarrow$ & \textsc{V\&T} $\uparrow$ & Params (M) $\downarrow$ \\
\Xhline{0.5\arrayrulewidth}
MultiBench range & $0.574-0.290$ & $93.3-93.6$ & $2.03-24.7$ \\
MultiBench SOTA & $0.290$ & $93.6$ & $2.03$ \\
\names & $\mathbf{0.201}$ & $\mathbf{96.5}$ & $4.18$ \\
\names\ multitask & $0.386$ & $\mathbf{96.1}$ & $\mathbf{1.00}$ \\
%\names\ multitask (large) & $\mathbf{0.245}$ & $\mathbf{96.0}$ & $2.11$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l|ccc|c}
\Xhline{3\arrayrulewidth}
Medium setting & \textsc{ENRICO} $\uparrow$ & \textsc{Push} $\downarrow$ & \textsc{AV-MNIST} $\uparrow$ & Params (M) $\downarrow$ \\
\Xhline{0.5\arrayrulewidth}
MultiBench range & $44.4-51.0$ & $0.574-0.290$ & $65.1-72.8$ & $21.2-51.7$ \\
MultiBench SOTA & $51.0$ & $0.290$ & $72.8$ & $21.30$ \\
\names & $\mathbf{52.6}$ & $\mathbf{0.278}$ & $70.4$ & $2.91$ \\
\names\ multitask & $\mathbf{53.1}$ & $\mathbf{0.287}$ & $70.4$ & $\mathbf{0.93}$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{2mm}

\begin{tabular}{l|cccc|c}
\Xhline{3\arrayrulewidth}
Large setting & \textsc{UR-FUNNY} $\uparrow$ & \textsc{MOSEI} $\uparrow$ & \textsc{MIMIC} $\uparrow$ & \textsc{AV-MNIST} $\uparrow$ & Params (M) $\downarrow$ \\
\Xhline{0.5\arrayrulewidth}
MultiBench range & $58.3-66.7$ & $76.4-82.1$ & $67.6-68.9$ & $65.1-72.8$ & $0.41-37.7$ \\
MultiBench SOTA & $66.7$ & $82.1$ & $68.9$ & $72.8$ & $9.86$ \\
%MultiBench SOTA $\le 0.53$M param & $63.2$ & $76.4$ & $68.9$ & $65.1$ &$0.43$M \\
\names & $63.3$ & $79.4$ & $67.7$ & $70.4$ & $2.11$ \\
\names\ multitask & $63.0$ & $79.9$ & $67.8$ & $70.4$ & $\mathbf{0.53}$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{-2mm}
\label{tab:multitask}
\end{table*}

==> 08_highmmt/tables/params.tex <==
\begin{table}[t]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Table of hyperparameters for multitask prediction on the \textbf{small} setting involving \textsc{Push}, \textsc{V\&T}: $2$ tasks in the same research area (robotics) but with different modality inputs: $\{ \textrm{image}, \textrm{force}, \textrm{proprioception}, \textrm{control} \}$ and $\{ \textrm{image}, \textrm{force}, \textrm{proprioception}, \textrm{depth} \}$ respectively, and readings come from different robot-dependent sensors.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}

\begin{tabular}{l|l|cc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{Part of Model} & \multirow{2}{*}{Hyperparameter} & \multicolumn{2}{c}{Values} \\ \cline{3-4} 
 &  & \multicolumn{1}{c}{\textsc{Push}} & \multicolumn{1}{c}{\textsc{V\&T}} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Unimodal Perceiver\\ Encoder\end{tabular}} & Depth & \multicolumn{2}{c}{1} \\ \cline{2-4} 
 & Num Latents & \multicolumn{2}{c}{20} \\ \cline{2-4} 
 & Latent Dim & \multicolumn{2}{c}{64} \\ \cline{2-4} 
 & Cross Attention Heads & \multicolumn{2}{c}{1} \\ \cline{2-4} 
 & Latent Self-Attention Heads & \multicolumn{2}{c}{8} \\ \cline{2-4} 
 & Cross Head Dim & \multicolumn{2}{c}{64} \\ \cline{2-4} 
 & Latent Head Dim & \multicolumn{2}{c}{64} \\ \cline{2-4} 
 & Num Latent Blocks Per Layer & \multicolumn{2}{c}{1} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Multimodal\\ Cross-Attention\\ Layer\end{tabular}} & Depth & \multicolumn{2}{c}{1} \\ \cline{2-4} 
 & Num Latents & \multicolumn{2}{c}{20} \\ \cline{2-4} 
 & Latent Dim & \multicolumn{2}{c}{64} \\ \cline{2-4} 
 & Cross Attention Heads & \multicolumn{2}{c}{1} \\ \cline{2-4} 
 & Latent Self-Attention Heads & \multicolumn{2}{c}{8} \\ \cline{2-4} 
 & Cross Head Dim & \multicolumn{2}{c}{64} \\ \cline{2-4} 
 & Latent Head Dim & \multicolumn{2}{c}{64} \\ \cline{2-4} 
 & Num Latent Blocks Per Layer & \multicolumn{2}{c}{1} \\ \hline
\begin{tabular}[c]{@{}l@{}}Classification Heads\\ (BatchNorm+Linear)\end{tabular} & Input/output dimensions & \multicolumn{1}{c}{756/32} & \multicolumn{1}{c}{1280/1} \\ \hline
\multirow{31}{*}{Training} & Optimizer & \multicolumn{2}{c}{Adam} \\ \cline{2-4}
 & Learning rate & \multicolumn{2}{c}{0.0005} \\ \cline{2-4}
 & Weight decay & \multicolumn{2}{c}{0.0} \\ \cline{2-4}
 & Training loss weights & \multicolumn{1}{c}{100.0} & \multicolumn{1}{c}{1.0} \\ \cline{2-4}
 & Batchsize & \multicolumn{1}{c}{18} & \multicolumn{1}{c}{64} \\ \cline{2-4}
 & Evaluation weights & \multicolumn{1}{c}{100.0} & \multicolumn{1}{c}{1.0} \\ \cline{2-4}
 & \begin{tabular}[c]{@{}l@{}}Original MultiBench\\ Input Dimensions\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 16x3\\Gripper Sensors: 16x7\\Image: 16x32x32\\Control: 16x7\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 128x128x3\\Force: 6x32\\Proprio: 8\\Depth: 128x128\\Action: 4\end{tabular}} \\ \cline{2-4} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input \\ Channel Size\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 3\\Gripper Sensors: 7\\Image: 1\\Control: 7\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 3\\Force: 32\\Proprio: 8\\Depth: 1\\Action: 4\end{tabular}} \\ \cline{2-4}
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input \\ Extra Axis\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 1\\Gripper Sensors: 1\\Image: 3\\Control: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 2\\Force: 1\\Proprio: 1\\Depth: 2\\Action: 1\end{tabular}} \\ \cline{2-4}
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input\\ Num\_freq\_bands\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 6\\Gripper Sensors: 6\\Image: 6\\Control: 6\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 6\\Force: 6\\Proprio: 6\\Depth: 6\\Action: 6\end{tabular}} \\ \cline{2-4}
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input\\ Max\_freq\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 1\\Gripper Sensors: 1\\Image: 1\\Control: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 1\\Force: 1\\Proprio: 1\\Depth: 1\\Action: 1\end{tabular}} \\ \cline{2-4}
 & Shared Modality Encoding & \multicolumn{2}{l}{N/A} \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{-4mm}
\label{params_small}
\end{table}

\begin{table}[t]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Table of hyperparameters for multitask prediction on the \textbf{medium} setting involving \textsc{AV-MNIST}, \textsc{ENRICO} and \textsc{PUSH}: $3$ tasks across $3$ domains (multimedia, HCI, and affective computing), again with vastly different modality sets: $\{ \textrm{image}, \textrm{audio} \}$, $\{ \textrm{image}, \textrm{set} \}$, and $\{ \textrm{image}, \textrm{force}, \textrm{proprioception}, \textrm{control} \}$ for  each task.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}

\begin{tabular}{l|l|clc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{Part of Model} & \multirow{2}{*}{Hyperparameter} & \multicolumn{3}{c}{Values} \\ \cline{3-5} 
 &  & \multicolumn{1}{c}{\textsc{AV-MNIST}} & \multicolumn{1}{c}{\textsc{ENRICO}} & \textsc{PUSH} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Unimodal Perceiver\\ Encoder\end{tabular}} & Depth & \multicolumn{3}{c}{1} \\ \cline{2-5} 
 & Num Latents & \multicolumn{3}{c}{12} \\ \cline{2-5} 
 & Latent Dim & \multicolumn{3}{c}{64} \\ \cline{2-5} 
 & Cross Attention Heads & \multicolumn{3}{c}{1} \\ \cline{2-5} 
 & Latent Self-Attention Heads & \multicolumn{3}{c}{8} \\ \cline{2-5} 
 & Cross Head Dim & \multicolumn{3}{c}{64} \\ \cline{2-5} 
 & Latent Head Dim & \multicolumn{3}{c}{64} \\ \cline{2-5} 
 & Num Latent Blocks Per Layer & \multicolumn{3}{c}{1} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Multimodal\\ Cross-Attention\\ Layer\end{tabular}} & Depth & \multicolumn{3}{c}{1} \\ \cline{2-5} 
 & Num Latents & \multicolumn{3}{c}{12} \\ \cline{2-5} 
 & Latent Dim & \multicolumn{3}{c}{64} \\ \cline{2-5} 
 & Cross Attention Heads & \multicolumn{3}{c}{1} \\ \cline{2-5} 
 & Latent Self-Attention Heads & \multicolumn{3}{c}{8} \\ \cline{2-5} 
 & Cross Head Dim & \multicolumn{3}{c}{64} \\ \cline{2-5} 
 & Latent Head Dim & \multicolumn{3}{c}{64} \\ \cline{2-5} 
 & Num Latent Blocks Per Layer & \multicolumn{3}{c}{1} \\ \hline
\begin{tabular}[c]{@{}l@{}}Classification Heads\\ (BatchNorm+Linear)\end{tabular} & Input/output dimensions & \multicolumn{1}{c}{128/10} & \multicolumn{1}{c}{128/20} & \multicolumn{1}{c}{768/2} \\ \hline
\multirow{22}{*}{Training} & Optimizer & \multicolumn{3}{c}{Adam} \\ \cline{2-5}
 & Learning rate & \multicolumn{3}{c}{0.001} \\ \cline{2-5}
 & Weight decay & \multicolumn{3}{c}{0.0} \\ \cline{2-5}
 & Training loss weights & \multicolumn{1}{c}{0.8} & \multicolumn{1}{c}{1.0} & \multicolumn{1}{c}{1.1} \\ \cline{2-5}
 & Batchsize & \multicolumn{1}{c}{32} & \multicolumn{1}{c}{32} & \multicolumn{1}{c}{32} \\ \cline{2-5}
 & Evaluation weights & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} \\ \cline{2-5}
 & \begin{tabular}[c]{@{}l@{}}Original MultiBench\\ Input Dimensions\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 28x28\\ Audio Spectogram:\\ 112x112\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 256x128x3\\ Set: 256x128x3 \end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 16x3\\Gripper Sensors: 16x7\\Image: 16x32x32\\Control: 16x7\end{tabular}}  \\ \cline{2-5} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input \\ Channel Size\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 16\\ (cut into 4x4 squares)\\ Audio Spectogram: 256\\ (cut into 16x16 squares)\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 3 \\ Set: 3 \end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 3\\Gripper Sensors: 7\\Image: 1\\Control: 7\end{tabular}}  \\ \cline{2-5} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input \\ Extra Axis\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 2\\ Audio Spectogram: 2\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 2\\ Set: 2\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 1\\Gripper Sensors: 1\\Image: 3\\Control: 1\end{tabular}} \\ \cline{2-5} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input\\ Num\_freq\_bands\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 6\\ Audio Spectogram: 6\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 6\\ Set: 6\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 6\\Gripper Sensors: 6\\Image: 6\\Control: 6\end{tabular}} \\ \cline{2-5} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input\\ Max\_freq\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 1\\ Audio Spectogram: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 1\\ Set: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Gripper Pos: 1\\Gripper Sensors: 1\\Image: 1\\Control: 1\end{tabular}}  \\ \cline{2-5} 
 & Shared Modality Encoding & \multicolumn{3}{l}{N/A} \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{-4mm}
\label{params_medium}
\end{table}



\begin{table}[t]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Table of hyperparameters for multitask prediction on the \textbf{large} setting involving \textsc{MIMIC}, \textsc{AV-MNIST}, \textsc{MOSEI} and \textsc{UR-FUNNY}: $4$ tasks across $3$ domains (healthcare, multimedia, and affective computing), again with vastly different modality sets: $\{ \textrm{time-series}, \textrm{table} \}$, $\{ \textrm{image}, \textrm{audio} \}$, and $\{ \textrm{text}, \textrm{video}, \textrm{audio} \}$ for the final $2$ tasks with different format of preprocessed embeddings of video and audio.\vspace{2mm}}
\setlength\tabcolsep{3.5pt}

\begin{tabular}{l|l|clll}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{Part of Model} & \multirow{2}{*}{Hyperparameter} & \multicolumn{4}{c}{Values} \\ \cline{3-6} 
 &  & \multicolumn{1}{c}{\textsc{MIMIC}} & \multicolumn{1}{l}{\textsc{AV-MNIST}} & \multicolumn{1}{l}{\textsc{MOSEI}} & \textsc{UR-FUNNY} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Unimodal Perceiver\\ Encoder\end{tabular}} & Depth & \multicolumn{4}{c}{1} \\ \cline{2-6} 
 & Num Latents & \multicolumn{4}{c}{20} \\ \cline{2-6} 
 & Latent Dim & \multicolumn{4}{c}{64} \\ \cline{2-6} 
 & Cross Attention Heads & \multicolumn{4}{c}{1} \\ \cline{2-6} 
 & Latent Self-Attention Heads & \multicolumn{4}{c}{6} \\ \cline{2-6} 
 & Cross Head Dim & \multicolumn{4}{c}{64} \\ \cline{2-6} 
 & Latent Head Dim & \multicolumn{4}{c}{64} \\ \cline{2-6} 
 & Num Latent Blocks Per Layer & \multicolumn{4}{c}{1} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Multimodal\\ Cross-Attention\\ Layer\end{tabular}} & Depth & \multicolumn{4}{c}{1} \\ \cline{2-6} 
 & Num Latents & \multicolumn{4}{c}{20} \\ \cline{2-6} 
 & Latent Dim & \multicolumn{4}{c}{64} \\ \cline{2-6} 
 & Cross Attention Heads & \multicolumn{4}{c}{4} \\ \cline{2-6} 
 & Latent Self-Attention Heads & \multicolumn{4}{c}{6} \\ \cline{2-6} 
 & Cross Head Dim & \multicolumn{4}{c}{64} \\ \cline{2-6} 
 & Latent Head Dim & \multicolumn{4}{c}{64} \\ \cline{2-6} 
 & Num Latent Blocks Per Layer & \multicolumn{4}{c}{1} \\ \hline
\begin{tabular}[c]{@{}l@{}}Classification Heads\\ (BatchNorm+Linear)\end{tabular} & Input/output dimensions & \multicolumn{1}{c}{128/2} & \multicolumn{1}{c}{128/10} & \multicolumn{1}{c}{384/2} & \multicolumn{1}{c}{384/2} \\ \hline
\multirow{22}{*}{Training} & Optimizer & \multicolumn{4}{c}{Adam} \\ \cline{2-6}
 & Learning rate & \multicolumn{4}{c}{0.0008} \\ \cline{2-6}
 & Weight decay & \multicolumn{4}{c}{0.001} \\ \cline{2-6}
 & Training loss weights & \multicolumn{1}{c}{1.2} & \multicolumn{1}{c}{0.9} & \multicolumn{1}{c}{1.1} & \multicolumn{1}{c}{1.5} \\ \cline{2-6}
 & Batchsize & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{40} & \multicolumn{1}{c}{32} & \multicolumn{1}{c}{32} \\ \cline{2-6}
 & Evaluation weights & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} \\ \cline{2-6}
 & \begin{tabular}[c]{@{}l@{}}Original MultiBench\\ Input Dimensions\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Static: 5\\ Timeseries: 24x12\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 28x28\\ Audio Spectogram:\\ 112x112\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 50x35\\ Audio: 50x74\\ Text: 50x300\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Image: 20x371\\ Audio: 20x81\\ Text: 50x300\end{tabular} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input \\ Channel Size\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Static: 1\\ Timeseries: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 16\\ (cut into 4x4 squares)\\ Audio Spectogram: 256\\ (cut into 16x16 squares)\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 35\\ Audio: 74\\ Text: 300\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Image: 371\\ Audio: 81\\ Text: 300\end{tabular} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input \\ Extra Axis\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Static: 1\\ Timeseries: 2\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 2\\ Audio Spectogram: 2\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 1\\ Audio: 1\\ Text: 1\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Image: 1\\ Audio: 1\\ Text: 1\end{tabular} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input\\ Num\_freq\_bands\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Static: 6\\ Timeseries: 6\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 6\\ Audio Spectogram: 6\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 3\\ Audio: 3\\ Text: 3\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Image: 3\\ Audio: 3\\ Text: 3\end{tabular} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}l@{}}Perceiver Input\\ Max\_freq\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Static: 1\\ Timeseries: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorless Image: 1\\ Audio Spectogram: 1\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Image: 1\\ Audio: 1\\ Text: 1\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Image: 1\\ Audio: 1\\ Text: 1\end{tabular} \\ \cline{2-6} 
 & Shared Modality Encoding & \multicolumn{4}{l}{The text modality from MOSEI and UR-FUNNY are shared.} \\
\Xhline{3\arrayrulewidth}
\end{tabular}

\vspace{-4mm}
\label{params_large}
\end{table}
